Simulations in statistical physics and biology: some applications

One of the most active areas of physics in the last decades has been that of critical phenomena, and Monte Carlo simulations have played an important role as a guide for the validation and prediction of system properties close to the critical points. The kind of phase transitions occurring for the Betts lattice (lattice constructed removing 1/7 of the sites from the triangular lattice) have been studied before with the Potts model for the values q=3, ferromagnetic and antiferromagnetic regime. Here, we add up to this research line the ferromagnetic case for q=4 and 5. In the first case, the critical exponents are estimated for the second order transition, whereas for the latter case the histogram method is applied for the occurring first order transition. Additionally, Domany's Monte Carlo based clustering technique mainly used to group genes similar in their expression levels is reviewed. Finally, a control theory tool --an adaptive observer-- is applied to estimate the exponent parameter involved in the well-known Gompertz curve. By treating all these subjects our aim is to stress the importance of cooperation between distinct disciplines in addressing the complex problems arising in biology. Contents: Chapter 1 - Monte Carlo simulations in stat. physics; Chapter 2: MC simulations in biology; Chapter 3: Gompertz equation

==> capitulodos.tex <==
\chapter{Monte Carlo Simulations in Biology}
\minitoc
%\bibliographystyle{plain}
\clearpage


\section{Proteins, DNA and Gene Expression}

Proteins are the complex molecules that make life possible. Keratin, essential in the structural conformation of our hair and nails,
is one among the many proteins used as supporting materials in biology. Cells are also made of proteins, and enzymes, which are responsible for
all chemical reactions inside living organisms, are proteins too. The information to produce the sequence of amino acids conforming certain protein
resides in the DNA molecule, making it of great importance for life.\\[1.5mm]
%
\indent A single strand of DNA is formed by unities named
nucleotides. Each nucleotide is composed by deoxyribose (a sugar
formed by five carbons), a phosphate group, and one of the four
possible nitrogenous bases: adenine (A), cytosine (C), guanine (G)
and thymine (G). Phosphodiester bridges link the phosphate group of
a nucleotide and the sugar of the next one, building in this way a
chain of nucleotides. The DNA molecule is formed when two of these
linear chains are joined by hydrogen bonds connecting the
nitrogenous bases standing out of the sugar-phosphate backbone of
each chain. All this chemical construction has a double helix
structure envisioned in 1952 by Cricks and Watson \cite{CW}. The
diameter of the helix is of 2 nm, and adjacent bases are separated
by 0.34 nm along the helix axis. Hence, the helix repeats itself
every 10 residues on each chain at intervals of 3.4 nm. Only
specific pairs of bases can form hydrogen bonds: the purine base A
always pairs with the pyrimidine base T through two hydrogen bonds,
and the other pyrimidine base C always pairs with the purine base G
this time by three hydrogen bonds \cite{dnapaisley}. A possible
explanation for this situation is that two purines require more than
2 nm for connection, which does not f\mbox{}it within the diameter
of the helix. On the other hand, there is too much space for two
pyrimidines to get close enough to form hydrogen bonds between them
\cite{basepair}. The rules of base pairing tell us that if we can
``read''  the sequence of nucleotides on one strand of DNA, we can
immediately infer the complementary sequence on the other strand.
Thus, DNA looks like a chemical code based on four letters, each one
corresponding to the four nitrogenous bases, aligned along a
double-helicoidal chain.
%\begin{figure}[h]
%\hfill
%\begin{minipage}[t]{6.8cm}
%\includegraphics[width=0.9\textwidth]{DNAt.ps}
%\end{minipage}
%\hfill
%\begin{minipage}[t]{5.2cm}
%\includegraphics[width=0.9\textwidth]{DNAt2.ps}
%\end{minipage}
%\hfill
%\caption{Structure of DNA.}
%\label{fig:DNA}
%\end{figure}\\[1.5mm]
%
\indent
At the same time, the genetic code is a universal translation table formed by three-bases words called codons. Each codon codifies for a specific
amino acid, so different sequences of codons build distinct proteins, and they can also build RNA molecules with a functional role.
One can obtain 64 distinct combinations mixing the four nitrogenous bases in clusters of three letters. This quantity is enough to code for
the 20 amino acids forming all proteins, and, as a matter of fact, almost all amino acids have more than one codon to codify them.
Three of these triplets are left apart to code for chain termination to release proteins at the end of their production process.
Moreover, one triplet is left as a signal to start the synthesis process. A segment of DNA sequence with the instructions to codify
for a functional product, protein or RNA, is named a gene, and the genome is the collection of all the ``recipes'' for the products that an
organism needs. The genome of a simple organism such as yeast has around 7,000 genes and the latest estimate for the human genome is of 25,000
genes \cite{genome}. It is important to stress that not all chain segments codify for proteins or RNA molecules: an overwhelming majority of
human DNA (98$\%$) contains non-coding regions (introns) that do not represent any particular functional product \cite{Domany}, although it
is believed that they help to protect the genes.\\[1.5mm]
%
\indent
Every cell of multicellular organisms has the entire set of information needed, but only some genes are expressed depending on the function
of the cell. For example, cells in our retina need photosensitive molecules, whereas our liver do not. {\bf A gene is expressed in a cell when
the protein or RNA it codes for is synthesized}. The large majority of abundantly expressed genes are associated with common functions, such as
metabolism, and hence are expressed in all cells. However, there will be differences in the expression profiles of different cells, and even in a
single cell, expression will vary with time, in a manner dictated by external and internal signals that reflect the state of the organism and
the cell itself \cite{Domany}.\\[1.5mm]
%
\indent
Although DNA molecule contains all the instructions to make a huge amount of diverse proteins, DNA is not able to come out of the eucaryotic cell
nucleus. Therefore, when certain protein is needed, another molecule called messenger RNA (m-RNA) is formed from DNA in a fundamental process called
transcription, and is this molecule who travels outside the nucleus carrying the information. RNA is also a nucleic acid but is formed by a single
 of nucleotides, and its sugar (ribose) is slightly different from deoxyribose. Besides, RNA has uracil U instead of the base thymine T. In cells,
 one can find three important types of RNA: messenger RNA (m-RNA), which transports the instructions to make a protein from the nucleus to the
 ribosomes, transfer RNA (t-RNA) which carries the amino acids to the ribosomes where the proteins are assembled and is found in the cytoplasm,
 and, finally, the r-RNA, or ribosomal RNA, which is one of the substances from what the ribosomes are made
 out \cite{ribosome}.\\[1.5mm]
%
\indent In the transcription process, the portion of DNA containing
the sequence for the needed product splits off, and then the free
RNA nucleotides existing in the nucleus are attached to the exposed
DNA nucleotides forming a complementary chain of RNA. This m-RNA
chain comes out of the nucleus carrying a complementary sequence and
arrives finally to the ribosome, where the sequence is translated
into a protein(translation process).
%\begin{figure}[h]
%\begin{center}
%\resizebox{100mm}{!}{\includegraphics{transcription.ps}}
%\caption{Transcription and translation processes in cells.}
%\label{fig:trans}
%\end{center}
%\end{figure}\\[1.5mm]
\indent
A cell may need a large number of some proteins and a small number of others, i.e. every gene may be expressed at a different level.
The manner in which the instructions to start and stop transcription are given for a certain gene is governed by regulatory networks.
Transcription is regulated by special proteins, called transcription factors, which bind to specific locations on the DNA, upstream from the
coding region. Their presence at the right site initiates or suppresses transcription. The basic paradigm of gene expression analysis states
that the biological state of a cell is reflected by its expression profile: the expression levels of all the genes of the genome. These in turn
are reflected by the concentrations of the corresponding m-RNA molecules \cite{Domany}.\\[1.5mm]
%
\indent Several genomes of diverse organisms have been completed in
the last years, the human genome, published on 2002, among them.
Now, the main focus is to understand the underlying function and
mechanisms behind these genomes. Some of the questions that remain
unanswered included what are the functional roles of different
genes, how genes are regulated, how do genes and gene products
interact, how does gene expression level differ in various cell
types and states, and how is gene expression changed by various
diseases or compound treatments\cite{Brazma}.

\section{DNA Microarrays}

Although m-RNA is not the ultimate product of a gene, transcription is the first step in gene regulation, and information about the transcript
levels is needed as a first approach for understanding gene regulatory networks. DNA microarrays or DNA chips are one of the latest breakthroughs
in experimental molecular biology precisely because they allow to monitor the expression of thousands of genes at the same time. The potential
 this technology is tremendous: monitoring gene expression levels in different developmental stages, tissue types, clinical conditions and
 different organisms can help understanding gene function and gene networks, assist in the diagnosis of disease conditions and reveal effects of
 medical treatments.\\[1.5mm]
%
\indent There are currently two main technologies that generate
large-scale gene expression data: cDNA and oligonucleotide
microarrays. CDNA microarrays contain large sets of complementary
DNA sequences several hundred bases long, each set representing a
gene, immobilized on a solid substrate. In oligonucleotide
microarrays, each gene is represented on the array by a set of 15-20
different oligonucleotide probes designed to hybridize perfectly to
some particular sequence, and some mismatch control
oligonucleotides, identical to the perfect match probes except for a
single base-pair mismatch. These mismatch control oligonucleotides
allow estimation of cross-hybridization, improving reproducibility
and accuracy of RNA quantification, and reducing the rate of
false-positives. In general, oligonucleotides used consist about
20-25 nucleotides, and are synthesized in situ with photolithography
techniques \cite{micrev}, \cite{micrev2}. In brief, functioning of
microarrays is based on the preferential binding of complementary
single stranded nucleic acid sequences, and a single microarray may
contain tens of thousands of spots.
%\begin{figure}[h]
%\hfill
%\begin{minipage}[t]{6.3cm}
%\includegraphics[width=0.9\textwidth]{Microarr1.ps}
%\end{minipage}
%\hfill
%\begin{minipage}[t]{5.1cm}
%\includegraphics[width=0.9\textwidth]{Microarr2.ps}
%\end{minipage}
%\caption{Hybridization on each spot of complementary DNA chains.}
%\label{fig:Microarr}
%\end{figure}\\[1.5mm]
%
\indent One of the most popular experiments involving cDNA
microarrays consists in compare m-RNA abundance in two samples. The
m-RNA molecules are extracted from cells taken from two tissues of
interest (e.g. tumour and normal tissues) \cite{Brown}. They are
reverse transcribed from RNA to DNA and their concentration is
enhanced. The resulting DNA is transcribed back into fluorescently
marked single strand RNA. For example, tumour tissue is labeled with
a red dye and normal tissue with a green one. The solution of marked
and enhanced m-RNA molecules (``targets'') that are copies of the
m-RNA molecules originally extracted from the tissue, is placed on
the chip and diffuses over the collection of single strand DNA
probes. When an m-RNA encounters a part of the gene of which it is a
perfect copy, it hybridizes to it with a high affinity (considerably
higher than with a bit of DNA of which it is not a perfect copy) and
when the m-RNA solution is washed off, only those molecules that
found their perfect match remain stuck to the chip. Next, the chip
is illuminated with a laser, and the stuck targets fluoresce. If RNA
from tumour tissue is in abundance, the spot will emit red light,
but if instead RNA from normal tissue is in abundance, it will
appear green. If tumour and normal RNA bind equally, the spot will
be yellow, while if neither binds, it will not fluoresce and appear
black \cite{Brazma}. Therefore, by measuring the light intensity
emanating from each spot, one obtains a measure of the number of
targets that stuck, which, in turn, is proportional to the
concentration of these m-RNA in the investigated tissues. CDNA
microarrays are a differential technique because only ratios between
both fluorescence wavelengths give meaningful information and hence,
only relative expressions levels are obtained. On the other hand,
with oligonucleotide arrays, absolute expression levels are measured
\cite{Moreau}.
%\begin{figure}[h]
%\begin{center}
%\resizebox{100mm}{!}{\includegraphics{microarray.ps}}
%\caption{Comparing normal and tumour gene expression levels with microarrays. Genes expressed only on tumour %tissue appear red, while genes expressed only on normal tissue appear green. If the gen is expressed equally %on both, the spot is yellow.}
%\label{fig:Microarray}
%\end{center}
%\end{figure}\\[1.5mm]
%
\indent The characterization of genes expressed differently in
normal and their corresponding tumour cells has been particularly
important \cite{Golub}. Arrays have also being used to discover
transcribed regions in genomic DNA \cite{Hughes}; to detect
polymorphism in copy number of regions of the genome\cite{Lucito},
which may be a new and important class of mutation; and to analyze
amplifications and deletions that are associated with oncogenic
transformation and some inherited conditions \cite{Anand},
\cite{Southern}. A number of diagnostic applications for arrays have
been suggested. The first to be granted approval by the US Food and
Drug Administration is the Roche AmpliChip for cytochrome P450. This
test will help doctors determine an individual's genotype to
determine appropriate drugs and doses to prescribe, minimizing
harmful drug reactions \cite{first}.

\section{Gene Clustering}

Microarray data analysis can be divided into two general classes: supervised and unsupervised analysis. The supervised approach assumes that for
 some (or all) profiles we have additional information, such as functional classes for the genes, or diseased/normal states attributed to the
 samples. We can viewed this additional information as labels attached to the rows or columns. Having this information, a typical task is to
 build a classifier able to predict the labels from the expression profile. If a clasiffier that is able to distinguish between two different,
 but morphologically closely related tumour tissues, can be constructed, such a classifier can be used for diagnosis. Classifiers are trained on a
 subset of data with a priori given classification and tested on another subset with known classification. After assessing the quality of the prediction they can be applied to data with unknown classif\mbox{}ication \cite{Brazma}. Unsupervised data analysis consists on clustering expression prof\mbox{}iles to f\mbox{}ind groups of co-regulated genes or related samples. An example of these two kind of clustering combined to predict clinical outcome of breast cancer can be seen at \cite{Veer}.

Some short DNA sequences in or around the gene, specifically in the promoter region, serve as switches that control gene expression.
Special proteins (transcription factors) interact with these binding sites, and represses or activates the transcription process of
the gene \cite{Moreau}. Various genes that share common functions or the same regulatory mechanism at the sequence level, can have the same
binding site sequence. As a result, similar expression patterns can correspond to similar binding site patterns. Then, a key step in the analysis
of gene expression data is the detection of groups of genes that exhibit similar behaviour of expression patterns (i.e. are coexpressed),
based on the idea that these genes share common regulatory or functional roles, assumption that has proved right in many experiments (see for
example \cite{Eisen}). \\[1.5mm]
%
\indent
The challenge is then transformed into the problem of clustering genes into groups based on their similarity in expression profiles. Instead
of clustering genes, experimental conditions can also be clustered, the task being now to find groups of experimental conditions (which can be,
for example, tumour samples) across which all the genes behave similarly. This type of clustering can be helpful for diagnosis. In gene expression,
elements to be clustered are usually genes and the vector of each gene is its expression pattern; similarity between genes can be measured in
various ways that are problem dependent, for example by the correlation coefficient between vectors. The goal is to partition the elements
into subsets, i.e. clusters, so that elements in the same cluster are highly similar to each other and elements from different clusters have low
similarity to each other.\\[1.5mm]
%
\indent
An essential step to obtain an effective cluster analysis is the preprocessing of the initial data. Although this work does not attempt to give a
detailed explanation of the various preprocessing steps, the most common ones are mentioned in the following. The first step is the normalization
of the hybridization intensities within a single experiment or across experiments. Besides, expression ratios are not symmetrical in the sense
that upregulated genes have expression ratios between one and infinity, while downregulated genes have expression ratios squashed between one
and zero. Taking the logarithms of these expression ratios results in symmetry between expression values of up- and downregulated genes.
This preprocessing step is called nonlinear transformation of the data. Other, but uncommonly used transformations, include square, square root,
and inverse transformations. Missing value replacement is another step, and is made only in the case of using a clustering algorithm that are not
able to handle missing values due to technical reasons in the data. Some genes do not really contribute to the biological process because their
expression values show little variation over the different experiments, and another problem are expression profiles with a considerable number of
missing values. This non desirable data is removed in the filtering process. Biologists are mainly interested in grouping gene expression
profiles that have the same relative behaviour, i.e. genes that are up- and downregulated together. Genes showing the same relative behaviour but
with diverging absolute behaviour will have a relatively high Euclidean distance, and cluster algorithms based on this distance measure will
therefore wrongfully assign the genes to different clusters. This can be prevented by applying standardization or rescaling to the gene expression
profiles so that they have zero mean and unit standard deviation. (\cite{Moreau}).\\[1.5mm]
%
\indent
In a typical experiment to monitor gene expression levels several DNA chips are used, and since each DNA chip contains thousands of spots, a
huge amount of information is obtained. These results are summarized in a $G \times S$ expression table, in which $G$ represents the number of
genes placed on every chip and $S$ is the number of DNA chips used (each chip accounting for different conditions, experiments, time points or
samples). Therefore, each row on this matrix corresponds to one particular gene and each column to a different sample. Each element $E_{gs}$ of the
matrix represents the expression level of gene $g$ in sample or condition $s$. Each column is called the profile of that condition, and each row
vector is the expression pattern of a gene across all the conditions, commonly named expression profile. If the input data for a clustering problem
is given in this form, it said to be as fingerprint data. Other type of input data is similarity data, where pairwise similarity values
between elements are used. These values can be computed from fingerprint data. Alternatively, the data can represent pairwise dissimilarity.
Fingerprints contain more information than similarity values, but the latter can be used to represent the input to clustering in any application.
Moreover, the fingerprint matrix is of order $G \times S$ while the similarity matrix is of order $G \times G$. It is important to note that in gene
expression applications typically $G >> S$, while in tissue classification applications often $G << S$ \cite{Sharan}.  \\[1.5mm]
%
\indent We need a way to measure the similarity (or distance)
between the genes or samples being compared and clustered. We can
regard these rows or columns in the matrix as points in
$n$-dimensional space or as $n$-dimensional vectors, where $n$ is
the number of samples for gene comparison, or number of genes for
sample comparison. The natural, so called Euclidean distance between
these points in the $n$-dimensional space may be the most obvious,
but not necessarily the best choice. There is no theory how to
choose the best distance measure. Possibly one right distance
measure in the expression profile space does not exist, and the
choice should depend on the problem studied \cite{Brazma}. Some
distance metrics commonly applied are the following:

\begin{enumerate}
\item Pearson correlation. The Pearson correlation $r$ is the dot product of two normalized vectors (i.e. the cosine between two vectors). It
measures the similarity in the shapes of two profiles, while not
taking the magnitude of the profiles into account, and therefore
suits well the biological intuition of coexpression.
\item Squared Pearson correlation. This is the square of the Pearson correlation, which considers two vectors pointing in the exact opposite
directions to be perfectly similar, which might also be interesting for biologists (because repression is a form of coexpression).
\item Euclidean distance. Euclidean distance measures the length of the straight line connecting the two points. It measures the similarity between
the absolute behaviours of genes, while the biologists are more interested in their relative behaviours. Thus, a standardization procedure is needed
before clustering using Euclidean distance. Importantly, after standardization, the Euclidean distance between two points $x$ and $y$ is related to
the Pearson correlation by $|x-y|^{2}=2(1-|r|)$.
\item Jackknife correlation. The jackknife correlation is an improvement for the Pearson correlation (which is not robust to outliers). Jackknife
correlation increases the robustness to single outliers by computing
a collection of all the possible leave-one-(experiment-)out Pearson
correlations between two genes and then selecting the minimum of the
collection as the final measure for the correlation.
\end{enumerate}

The first generation of cluster algorithms used for gene expression
profiles were developed for purposes did not related with biological
research (e.g. hierarchical clustering, K-means and self organizing
maps(SOM)). Although it is possible to obtain biologically
meaningful results with these algorithms, some of their
characteristics often complicate their use for clustering expression
data. More recently, new algorithms have been developed specifically
for gene expression profile clustering to overcome some of the
limitations of earlier methods. These algorithms include, among
others, model-based algorithms, the self-organizing tree algorithm
(SOMA), quality-based algorithms, and biclustering algorithms. Also,
some procedures have been developed to help biologists estimate some
of the parameters needed for the first generation of algorithms,
such as the number of clusters present in the data. While it is
impossible to give an exhaustive description of all clustering
algorithms developed for gene expression data, we try here to
illustrate some of them.

\subsection{Hierarchical Clustering}

Agglomerative or hierarchical clustering algorithms (\cite{Lance}) are among the oldest and most widely used clustering methods applied to gene
expression data. Typically, the algorithm takes each expression profile as one cluster at the beginning. Then computes the distance between every
pair of clusters, and the pair of clusters with the minimum distance is merged; the procedure is carried on iteratively until all elements ends into
one single cluster. The whole clustering process is presented as a tree called a dendrogram and the original data are often reorganized in a heat map
demonstrating the relationships between genes or conditions. After the full tree is obtained, the determination of the final clusters is achieved by
cutting the tree at a certain level or height, which is equivalent to putting a threshold on the pairwise distance between clusters. The decision of
the final clusters is arbitrary, because it is difficult to predict which level will give the best biological results. Note that the memory
complexity of hierarchical clustering is quadratic in the number of gene expression profiles, which can be a problem due to the large number of
genes involved in experiments.\\[1.5mm]
%
\indent As in every step of agglomerative clustering, the two
subsets that are closest or more similar to each other are merged,
the distance between two clusters has to be defined. There are four
common options:

\begin{enumerate}
\item Single linkage. The distance between two clusters is taken as the distance between the two closest data points, each point belonging to a
different cluster.
\item Complete linkage. The distance between the two furthest data points, each one in a different cluster.
\item Average linkage. Both single linkage and complete linkage are sensitive to outliers. Average linkage provides an improvement by defining the
distance between two clusters as the average of the distances between all pairs of points in the two clusters.
\item Ward's method. At each step of agglomerative clustering, instead of merging the two clusters that minimize the pairwise distance between
clusters, Ward's method (\cite{Ward}) merges the two clusters that
minimize the ``information loss'' for the step. The ``information
loss'' is measured by the change in the sum of squared error of the
clusters before and after the merge. In this way, Ward's method
assesses the quality of the merged cluster at each step of the
agglomerative procedure.
\end{enumerate}

These methods yield similar results if the data consist of compact and well separated clusters. However, if some of the clusters are close to
each other or if the data have a dispersed nature, the results can be quite different. Ward's method, although less well known, often produces the
most satisfactory results \cite{Sheng}.\\[1.5mm]
%
\indent
Eisen et al. developed a clustering software package based on average linkage hierarchical clustering \cite{Eisen}. The clustering program is
called Cluster, and the accompanying visualization program is called TreeView. Both programs are available at
http://rana.lbl.gov/EisenSoftware.htm.

\subsection{K-Means Clustering}

K-means clustering (\cite{Hartigan}, \cite{Tavazoie}) is a simple
and popular partitioning method for data analysis. The number of
clusters K in the data is needed as an input for the algorithm.
K-means starts by assigning at random all gene expression profiles
to one of the K clusters. Iteratively, the center, which is nothing
more than the average expression vector of each cluster, is
calculated and then the gene expression vectors are reassigned to
the cluster with the closest cluster center. The initial mean
vectors are called the seeds. The iterative procedure converges when
all the mean vectors of the clusters remain stationary or the given
number of iterations is exceeded. Since it is difficult to predict
the number of clusters in advance, the predefinition of the number
of clusters by the user is arbitrary. In practice, this implies the
use of a trial-and-error approach where a comparison and biological
validations of several runs of the algorithm with different
parameter settings are necessary (\cite{Moreau}). Another parameter
that influence the result of K-means clustering is the choice of the
seeds. The algorithm suffers from the problem that with different
seeds the algorithm can yield very different result.

\subsection{Self-Organizing Maps}

SOM (\cite{Kohonen}) is a technique developed by Kohonen for fitting a number of reference vectors to the distribution of gene data, by means of a
set of nodes. The nodes are the intersections of a two-dimensional grid (usually of hexagonal or rectangular geometry). In the high-dimensional
input space (with the gene expression vectors), each node represents a reference vector (similar to the mean vectors in the K-means algorithm).
The dimension of the grid (e.g. lattice of 6x5 nodes) needs to be specified a priori. The initial position of the reference vectors is randomly
chosen, and then the algorithm selects a random data vector $p$, identifies the node $n_p$ whose reference vector is closest to $p$, and updates
the position of all reference vectors towards $p$ according to a predefined learning function. The amount of position adjustment determined by the
learning function decreases as the distance between $n$ and $n_p$ (in the grid) and the iteration number grow. The intuition for this learning
process is that the reference vectors that are close enough to $p$ will be pulled towards it, and the stiffness of the grid structure will propagate
some of impact to neighbouring nodes. As a result, a reference vector is pulled more towards input vectors that are closer to the reference vector
itself and is less influenced by the input vectors located further away. In the meantime, this adaptation procedure of reference vectors is
reflected on the output nodes (nodes associated with similar reference vectors are pulled closer together on the output grid). The algorithm
terminates when convergence of the reference vectors is achieved or after completing a pre-defined number of training iterations.\\[1.5mm]
%
\indent
Because of the advantage in visualization, choosing the geometry of the output grid is not as crucial a problem as the choice of the number of
clusters for a K-means method. Like the K-means method, the initial choice of reference vectors remains a problem that influences the final
clustering result of SOM clustering. A good way to seed the reference vectors is to use the result from a principal component
analysis(PCA) \cite{Sheng}.\\[1.5mm]
%
\indent
Tamayo et al. \cite{Tamayo} devised a gene expression clustering software, GeneCluster, which uses the SOM algorithm. The software is
available at \\ http://www.broad.mit.edu/cancer/software/genecluster2/gc2.html.

\subsection{Self-Organizing Tree Algorithm}

SOTA combines SOM and hierarchical clustering techniques. As in SOM, SOTA maps the input gene profiles to an output space of nodes. However,
the nodes in SOTA, instead of being in a two-dimensional grid, are in the topology (or geometry) of a binary tree. The number of nodes in
SOTA is not fixed from the beginning (in contrast to SOM) because the tree structure of the nodes grows during the clustering procedure.\\[1.5mm]
%
\indent The initial system is composed of two external elements,
denoted as cells, connected by an internal element that its called
node, like a tree with two leaves. Each cell (or node) is a
reference vector with the same size as the gene profiles. In the
beginning, the entries of the
two cells and the node are randomly initialized. The series of operations performed until a cell generates two descendants is called a cycle.
During a cycle, cells and nodes are repeatedly adapted by the input gene profiles. Adaptation in each cycle consists on the presentation of all
expression profiles to the network, and this implies two steps: first, each gene profile is associated with the cell whose reference vector is
located closest to it, and second, the reference vector of this cell and its neighbouring nodes, including its parent node and its sister cell,
are updated based on some neighbourhood weighting parameters (which perform the same role as the neighbourhood function in SOM). Thus, a cell is
moved into the direction of the expression profiles that are associated with it. The network follows its growing process by replicating the cell
whose associated profiles exhibits the highest heterogeneity, i.e., the largest variability (defined by the maximal distance between two profiles
that are associated with the same cell). This cell gives rise to two new descendants cells and become a node. The values of the two new cells are
identical to the node that generate them and the whole procedure starts again. The growing process ends when the heterogeneity of the system falls
below a threshold. This threshold can be set to zero for a fully resolved dendogram similar to that provided by hierarchical clustering. If the
threshold is obtained from the randomized distribution of data, SOTA will provide the cluster hierarchy that minimizes the probability of having
missassigned genes to them \cite{Herrero}.\\[1.5mm]
%
%\indent
%To obtain a statistical definition for this threshold a randomized version of the entire data set is used (for %each expression profile all its expression values are randomly and independently shuf\mbox{}f\mbox{}led--this operation %destroys the actual correlation between expression prof\mbox{}iles) and the distances between all possible pairs of gene %expression prof\mbox{}iles in this version of the data are calculated. This results in the probability distribution of %the distances that could occur by chance (i.e. the distribution that described the probability that two unrelated %expression prof\mbox{}iles have a certain distance). The threshold of variability can now be def\mbox{}ined by choosing a %conf\mbox{}idence level alpha (e.g., alpha=5\%), so that only a fraction alpha of the randomized gene expression %prof\mbox{}iles have a distance smaller than this threshold. Using this threshold ensures that the fraction of wrong %assignments (unrelated prof\mbox{}iles assigned to the same cluster) in the actual cluster result is limited by the %alpha value.\\[1.5mm]
%
\indent SOTA has two crucial advantages: the topology is that of a
hierarchical tree, and the clustering obtained is proportional to
the heterogeneity of the data, instead of the number of items (this
is due to the fact that SOTA is distribution preserving while SOM is
topology preserving). In both SOM and SOTA, the training process
changes the vectors in the nodes to weighted averages of the gene
expression patterns associated to them. The advantage in the case of
SOTA is that the binary topology produces a nested structure in
which nodes at each level are averages of items below them (items
that can be nodes or in the case of terminal nodes, genes). This
makes it straightforward to compare average patterns of gene
expression at different hierarchical levels even for large data sets
\cite{Herrero}.

\subsection{Model Based Clustering}

Model Based Clustering assumes that the data are generated by a
finite mixture of underlying probability distributions such as
multivariate normal distributions. In this case, each cluster $C_i$
is represented by a multivariate Gaussian model $p_i$ in $d$
dimensions:
\begin{equation}
p_{i}(y_{j}|\mu_{i},\sum_{i})= \frac{1}{(2 \pi)^{d/2}
|\sum_{i}|^{d/2}}e^{-1/2(y_j-\mu_{i})^{T}(\sum_{i})^{-1}(y_j-\mu_{i})},
\end{equation}
where $y_j$ is an expression profile and $\mu_{i}$ and $\sum_{i}$
the mean and covariance matrix of the multivariate normal
distribution respectively \cite{Moreau}.

The covariance matrix $\sum_{i}$ can be represented by its
eigenvalues decomposition, which in general takes the following
structure:
\begin{equation}
\sum_{i} = \lambda_{i} D_{i} A_{i} D_{i}^{T},
\end{equation}
where $D_{i}$ is the orthogonal matrix of the eigenvectors of
$\sum_{i}$, $A_{i}$ is a diagonal matrix whose elements are
proportional to the eigenvalues of $\sum_{i}$, and $\lambda_{i}$ is
the constant of proportionality. This decomposition implies a nice
geometric interpretation of the clusters: $D_{i}$ controls the
orientation, $A_{i}$ controls the shape, and $\lambda_{i}$ controls
the volume of the cluster. Note that simpler forms of the covariance
structure can be used (e.g., by having some of the parameters take
the same values across clusters), thereby decreasing the number of
parameters that have to be estimated but also decreasing the model
flexibility (capacity to model more complex data structures).

The mixture model $p$ itself takes then the following form:
\begin{equation}
p(y_{j})= \sum_{i=1}^{K} \pi _{i} p_{i}(y_{j}|\mu _{i}, \sum_{i}),
\end{equation}
where $K$ is the number of clusters and $\pi _{i}$ is the prior
probability that an expression profile belongs to cluster $C_{i}$ so
that:
\begin{equation}
\sum_{i=1}^{K} \pi_{i}=1.
\end{equation}

In practice we would like, given a collection of expression profiles $y_{j}(j=1,...,n)$, to estimate all the
parameters ($\pi_{i}, \mu_{i}, \sum_{i} (i=1,...,K)$, and $K$ itself) of this mixture model. In a first
step $\pi_{i}, \mu_{i}, \sum_{i} (i=1,...,K)$ are estimated with an EM algorithm using a fixed value for $K$ and a fixed covariance
structure \cite{Moreau}. In the EM algorithm, the Expectation steps and Maximization steps alternate. In the E step, the probability of each
observation belonging to each cluster is estimated conditionally on the current parameter estimates. In the M step the model parameters are
estimated given the current group membership probabilities. When the EM algorithm converges, each observation is assigned to the group with the
maximum conditional probability \cite{Yeung}. This parameter estimation is then repeated for different values for $K$ and different covariance
structures. The result is thus a collection of different models fitted to the data and all having a specific value for $K$ and a specific covariance
structure. In a second step the best model in this group of models is selected (i.e., the most appropriate number of parameters and a covariance
structure is chosen here). This model selection step involves the calculation of the Bayesian Information Criterion (BIC) for each model \cite{Schwarz}, which is not further discussed here.\\[1.5mm]
%parameters
\indent A good implementation for model based clustering (called
MCLUST) is available at\\ www.stat.washington.edu/fraley/mclust.
Yeung et al. reported good results using this software on several
synthetic data sets and real expression data sets. McLachlan et al.
\cite{McLachlan} have also implemented model-based clustering in a
Fortran program called EMMIX, which is also freely available from
the web at http://www.maths.uq.edu.au/\~gjm/emmix/EMMIX.f.

\subsection{Quality-Based Algorithms}

Quality-based algorithms produces clusters with a quality guarantee that ensures that all members of a cluster are coexpressed (this property is
called transitivity). This concept was introduced by Heyer, Kruglyak and Yooseph, (\cite{Heyer}) and their implementation is called QT \_ Clust.
The quality of a cluster $C$ is defined as a diameter (equal to $1 - min_{i}, j \in s_{ij}$, where $s_{ij}$ is the jackknife correlation between
expression profiles $i$ and $j$), but the method can be easily extended to other definitions.\\[1.5mm]
%
\indent
The algorithm considers every expression profile in the data set as a cluster seed (one could also call this a cluster center) and iteratively
assigns the expression profiles to these clusters that cause a minimal increase in diameter until the diameter threshold, i.e., quality guarantee,
is reached. Note that at this stage every expression profile is made available to every candidate cluster and that there are as many candidate
clusters as there are expression profiles. At this point, the candidate cluster that contains the most expression profiles is selected as a valid
cluster and removed from the data set where after the whole process starts again. The algorithm stops when the number of points in the largest
remaining cluster falls below a threshold. Note that this stop criterion implies that the algorithm will terminate before all expression
profiles are assigned to a cluster.\\[1.5mm]
%
\indent This approach has some advantages, for example it is
possible to find clusters containing highly coexpressed genes, and
these clusters might therefore be good seeds for further analysis.
Moreover, genes not really coexpressed with other members of the
data set are not included in any of the clusters. Some disadvantages
are that the quality guarantee of the clusters is a user defined
parameter hard to estimate, it is hard to use by biologists, needs
extensive parameter fine-tuning, and produces clusters all having
the same fixed diameter not optimally adapted to the local data
structure \cite{Moreau}.

\subsection{Adaptive Quality-Based Clustering}

Adaptive quality-based clustering (\cite{DeSmet}) consist of a two-step approach. In the first step, a quality-based approach is performed to
locate a cluster center in an area where the density of gene expression profiles is locally maximal using a preliminary estimate of the radius
(i.e. the quality) of the cluster. In the second step, called adaptive step, the algorithm re-estimates the radius of the cluster so that the genes
belonging to it are, in a statistical sense, significantly coexpressed. To this end, a bimodal and one-dimensional probability distribution (the
distribution consists of two terms: one for the cluster and one for the rest of the data) describing the Euclidean distance between the data points
and the cluster center is fitted to the data using an expectation-maximization (EM) algorithm.\\[1.5mm]
%
\indent
Finally, step one and two are repeated, using the re-estimation of the quality as the initial estimate needed in the first step, until the
relative difference between the initial and re-estimated quality is sufficiently small. The cluster is subsequently removed from the data and the
whole procedure is restarted. Note that only clusters whose size exceeds a predefined number are presented to the user.\\[1.5mm]
%
\indent
In adaptive quality-based clustering, users have to specify a threshold for quality control. This parameter has a strict statistical meaning and is
therefore much less arbitrary (in contrast to the case in QT\_Clust). It can be chosen independently of a specific data set or cluster and it allows
for a meaningful default value (95\%) that in general gives good results. This makes the approach user friendly without the need for extensive
parameter fine-tuning. Furthermore, with the ability to allow the clusters to have different radius, adaptive quality-based clustering produces
clusters adapted to the local data structure\cite{Moreau}. An application of Adaptive Quality- Based Clustering to nervous system is found
in \cite{Wen}.\\[1.5mm]
%
\indent
However, the method has some limitations like it does not converge in every situation. A server running the program is available
at http://homes.esat.kuleuven.be/\~thijs/Work/Clustering.html

\subsection{Biclustering and Some Physics Related Algorithms}

Clustering can be applied to either the rows or the columns of the data matrix, separately. Biclustering, on the other hand, performs
clustering in these two dimensions simultaneously. This means that clustering derives a global model while biclustering produces a local
model\cite{Madeira}. The term biclustering was first used by Cheng and Church \cite{Cheng} in gene expression data analysis. It refers to a
distinct class of clustering algorithms that perform simultaneous row-column clustering. One of the earliest biclustering formulations is the
direct clustering algorithm introduced by Hartigan \cite{Hartigan}, also known as block clustering.\\[1.5mm]
%
\indent
The goal of biclustering techniques is thus to identify subgroups of genes and subgroups of conditions, by performing simultaneous clustering
of both rows and columns of the gene expression matrix, instead of clustering these two dimensions separately. We can then conclude that, unlike
clustering algorithms, biclustering algorithms identify groups of genes that show similar activity patterns under a specific subset of experimental
conditions \cite{Madeira}.\\[1.5mm]
%
\indent
There are also several physics related clustering algorithms, e.g. Deterministic Annealing \cite{Rose} and Coupled Mass \cite{Angelini}.
Deterministic
Annealing uses the same cost function as K-means, but rather than minimizing it for a fixed value of clusters K, it performs a statistical
mechanics type analysis, using a maximum entropy principle as its starting point. The resulting free energy is a complex function of the
number of centroids and their locations, which are calculated by a minimization process. This minimization is done by lowering the temperature
variable slowly and following minima that move and every now and then split (corresponding to a second order phase transition). Since it has been
proven \cite{Schneider} that in the generic case the free energy function exhibits first order phase transitions, the deterministic annealing
procedure is likely to follow one of its local minima \cite{Domany}.\\[1.5mm]
%
\indent Finally, it is important to stress that clustering methods
have been used in a large variety of scientific disciplines and
applications that include pattern recognition \cite{Duda}, learning
theory \cite{Moody}, astrophysics \cite{Dekel}, medical images and
data processing \cite{Phillips}, machine translation of text
\cite{Cranias}, satellite data analysis \cite{Baraldi}, as well as
speech recognition \cite{Kosaka}. %\clearpage

\section{Superparamagnetic Gene Clustering: Monte Carlo Simulations}

This method takes the data points generated by gene expression profiles as sites of an inhomogeneous Potts ferromagnet, and was first proposed
by Eytan Domany et al. \cite{BDomany}. The presence of clusters in the data gives rise to magnetic grains, and working in the
superparamagnetic phase, the SPC algorithm decides if a data point belong to the same grain using the pair correlation function of the
Potts spins. Additionally, temperature controls the level of resolution obtained.\\[1.5mm]
%
\indent
A Potts system is said to be homogeneous when its spins are on a lattice and all nearest neighbour couplings are equal, $J_{ij} = J$. This system
exhibits two phases, at high temperatures is paramagnetic or disordered, and at low temperatures is ordered. In the disordered phase the
correlation function $G_{ij}$ decays to $1/q$ when the distance between points $v_i$ and $v_j$ is large (remember from last chapter, that $q$ is
the number of possible states in the Potts model). This is the probability to find two completely independent Potts spins in the same state.
At very high temperatures even neighbouring sites have $G_{ij} \approx 1/q$. As the temperature is lowered, the system undergoes a sharp transition
to an ordered, ferromagnetic phase, meaning that one Potts state dominates the system. At very low temperatures $G_{ij} \approx 1$ for all
pairs ${v_i, v_j}$, i.e. all spins have the same $q$ \cite{Domany98}.\\[1.5mm]
%
\indent In strongly inhomogeneous Potts models, spins form magnetic
grains with very strong couplings between neighbours that belong to
the same grain, and very weak interactions between all other pairs.
At low temperatures such a system is also ferromagnetic, but as the
temperature is raised the system may exhibit an intermediate,
super-paramagnetic phase. In this phase strongly coupled grains are
aligned (i.e. are in their respective ferromagnetic phases), while
there is no relative ordering of different grains. This is
illustrated in Fig. \ref{fig:SP}.
\begin{figure}[h]
\begin{minipage}[t]{5.5cm}
\includegraphics[width=0.9\textwidth]{ferrodes1.eps}
\end{minipage}
\begin{minipage}[t]{5.5cm}
\includegraphics[width=0.9\textwidth]{ferrosp1.eps}
\end{minipage}
\begin{minipage}[t]{5.5cm}
\includegraphics[width=0.9\textwidth]{ferrop1.eps}
\end{minipage}
\caption{At high T all sites have different spin values, but as T is
lowered, regions of aligned spins appears (superparamagnetic phase).
At low T, the system is completely ordered.} \label{fig:SP}
\end{figure}\\[1.5mm]
%
\indent
At the transition temperature from the ferromagnetic to super-paramagnetic phase a pronounced peak of $\chi$ is observed \cite{BDomany}. As the
temperature is further raised, the super-paramagnetic to paramagnetic transition is reached; each grain disorders and $\chi$ abruptly diminishes
by a factor that is roughly the size of the largest cluster. Thus the temperatures where a peak of the susceptibility occurs and the temperatures at
which $\chi$ decreases abruptly indicate the range of temperatures in which the system is in its super-paramagnetic phase. In principle, one can
have a sequence of several transitions in the super-paramagnetic phase: as the temperature is raised the system may break first into two clusters,
each of them in turn breaks into more (macroscopic) sub-clusters and so on. Such a hierarchical structure of the magnetic clusters reflects a
hierarchical organization of the data into categories and sub-categories \cite{WDomany}.\\[1.5mm]
%
\indent
In concreteness, SPC method consists on three stages. First, to specify the Hamiltonian which governs the system. Second, find the temperature range
where the superparamagnetic phase take place, taking into acount the susceptibility behaviour. Finally, the correlation of neighbouring pairs of
spins, $G_{ij}$ is measured and, taking into account these values, the clusters are formed.\\[1.5mm]
%
\indent
\subsection{Detailed Description of SPC}

Each expression profile is represented as a point in a $D$ dimensional space, and a random spin value $\sigma_{i}$, $i=1,2,...,q$ is assigned to
it. A small value $q$ hinders the identification of the SPM clusters since different clusters are then forced to point into the same Potts
direction. Too large $q$ makes the calculations more cumbersome. However, the results depend only weakly on the value of $q$. In the next step,
the neighbours of each spin $v_i$ are calculated using the $K$ mutual neighbour criterion. This criterion initially calculates the $K$ nearest
points of each site. If $v_i$ has $v_j$ among its $K$ nearest points, and $v_j$, in turn, has $v_i$ as one of its $K$ nearest points, then $v_i$
and $v_j$ are considered as neighbours.\\[1.5mm]
%
\indent The average number of neighbours $\hat K$ and the average of
all distances $a$ between neighbouring pairs $v_i$ and $v_j$ are
then computed, and finally the interaction couplings which will
appear in the Hamiltonian will be calculated as follows:

\begin{equation}\label{eq:js}
J_{ij}= \left\{ \begin{array}{ll}
\frac{1}{\hat K}e^{-\frac{d_{ij}^2}{2a^2}} & \textrm{if $v_i$ and $v_j$ are neighbours}\\
\\
0 & \textrm{otherwise}
\end{array} \right.
\end{equation}

Choosing $J_ij$ in this way creates strong interactions between spins associated with the data from high density regions, and weak interactions
between neighbours that are in low density regions \cite{Barad}.\\[1.5mm]
%
\indent Any different assignment of spins to data points $S$ has an
energy cost given by:

\begin{equation}\label{eq:ha}
H(S)= \sum_{i,j} J_{ij} \delta_{\sigma_i,\sigma_j} ,
\end{equation}
where the sum is over neighbouring sites. The function $\delta_{\sigma_i,\sigma_j}$ is the Kroenecker symbol taking the value $1$
when $\sigma_i=\sigma_j$ and $0$ otherwise. The lowest possible energy cost, $H({S}) =0$ is attained when we assign the same spin to all
points, which corresponds to all data points being assigned to the same cluster. Moreover, as one chooses interactions that are a decreasing
function of the distance $d_{ij}$, then the closer two points are to each other, the more likely is for them to be in the same state. In
summary, this Hamiltonian procedure penalizes placing spins at points $i,j$ in different clusters, and this penalty decreases with the distance
between the points \cite{WDomany}.\\[1.5mm]
%
\indent
The next step is the calculation of magnetization, susceptibility and correlation function for pairs of neighbours $G_{ij}$ over a range of
temperatures using Monte Carlo technique. The original creators of SPC used the Swendsen Wang algorithm.\\[1.5mm]
%
\indent
As the temperature increases, $M$ varies from $1$ to $0$ via sharp phase transitions. At low temperatures the system is fully magnetized and
the fluctuations in $m$ are negligible. As $T$ increases to the point where the single cluster breaks into subclusters (or
become completely disordered), fluctuations become very large. Hence, one expect to identify the transitions at which clusters break up by the
sharp peaks of the susceptibility \cite{EDomany}.\\[1.5mm]
%
\indent
The strategy is to vary $T$ and measure $\chi(T)$. Transitions show up as peaks of $\chi$. At temperatures between transitions, we
expect to observe relatively stable phases that correspond to some clusters being ordered internally and uncorrelated with other clusters.
Within each such phase, $G_{ij}$ is measured. The value of $G_{ij}$ is the probability to find the two Potts spins $\sigma_i$ and $\sigma_j$ in the
same state, i.e. the probability to find them in the same cluster. By the relation to granular ferromagnets we expect that the distribution
of $G_{ij}$ is bimodal; if both spins belong to the same ordered grain (cluster), their correlation is close to 1; if they belong to two clusters
that are not relatively ordered, the correlation is close to 0. Rather than thresholding the distances between pairs of points to decide their
assignment to clusters, we use the pair correlations, which reflect a collective aspect of the data's distribution \cite{WDomany}.\\[1.5mm]
%
\indent Clusters are identified in three steps:
\begin{enumerate}
\item Build the cores of the clusters using a thresholding procedure. If $G_ij > 0.5$, a link is set between the neighbour data
points $v_i$ and $v_j$. The resulting connected graph depends weakly in the value used in this thresholding, as long as it is bigger
than $1/q$ and less than $1-2/q$ \cite{WDomany}. The reason is that the distribution of the correlations between two neighbouring spins peaks
strongly at these two values and is very small between them.
\item Capture points lying in the periphery by linking each point to its neighbour of maximal correlation. Of course, some points were already
linked in step one.
\item Data clusters are identified as the linked components of the graph obtained in the previous steps.
\end{enumerate}

The temperature controls the resolution at which the data are clustered.

It is intuitively clear that if a set of data points form a dense
cloud, isolated from the rest of the data, the corresponding spins
will form a ferromagnetic domain at some low temperature, which will
become paramagnetic and lose its correlations only at a high
temperature. Hence the size of the temperature interval $dT$ in
which such a ferromagnetic domain exists can be used as a measure of
the stability and significance of the corresponding data cluster.

Some of the demonstrated useful properties of SPC are the following: (a) the number of clusters is determined by the algorithm itself and not
externally prescribed (as is done by SOM and K-means); (b) presents stability against noise; (c) generates a hierarchy (dendrogram) and
provides a mechanism to identify in it robust, stable clusters (by the value of dT ); (d) ability to identify a dense set of points forming a
cloud of an irregular (non-spherical shape) as a cluster \cite{Domany}.\\[1.5mm]
%
\indent The SPC method has been used in various contexts, like
computer vision \cite{Gdalyahu}, speech recognition \cite{WDomany}
and identification of clusters of companies in stock indices
\cite{Kullmann}. Its first direct application to gene expression
data has been for analysis of the temporal dependence of the
expression levels in a synchronized yeast culture \cite{Getz},
identifying gene clusters whose variation reflects the cell cycle.
Subsequently, the SPC was used to identify primary targets of p53
\cite{Kannan}, the most important tumour suppressor that acts as a
transcription factor of central importance in human cancer. SPC has
been used also to cluster protein sequences \cite{Tetko}, and to
classify or identify new genes associated with colon and skin cancer
\cite{Gal}.

\subsection{Future Directions}

The location of the superparamagnetic phase in the SPC algorithm is
closely related to the phase transitions occurring in the system.
The introduction of the Wolff algorithm instead of the originally
used Swendsen-Wang algorithm will probably improve the efficiency of
the method, and this is left for future investigations, as well as a
comparison of different methods with the SPC algorithm.


==> capitulotres.tex <==
\chapter{Gompertz Equation}
\minitoc
%\bibliographystyle{plain}
\clearpage

%\documentclass{article}

%\usepackage[english]{babel}
%\usepackage{eufrak,euscript,latexsym}
%\usepackage{fancyhdr,exscale,color}

%\usepackage{amsmath}
%\usepackage{graphics}
%, amsthm}
%\begin{document}

%\pagenumbering{arabic}

\hyphenation{ge-ne-ral}
\hyphenation{se-xual}
\hyphenation{re-cu-pe-ra-ti-ve}
\hyphenation{scien-ti-fic}
\hyphenation{ne-ce-ssa-ry}
\hyphenation{ho-meos-ta-tic}
\hyphenation{Tran-sac-tions}
\hyphenation{in-su-ran-ce}
\hyphenation{geo-me-tri-cal}
\hyphenation{si-mi-lar}
\hyphenation{ob-ser-ving}
\hyphenation{pu-bli-shed}
\hyphenation{pa-tterns}
\hyphenation{des-troy}
\hyphenation{lo-ga-rithms}
\hyphenation{co-rres-pon-ded}
\hyphenation{des-cri-be}
\hyphenation{mor-ta-li-ty}

\hyphenation{Not-with-stan-ding}
\hyphenation{de-via-tion}
\hyphenation{a-no-ther}
\hyphenation{appro-xi-ma-te-ly}
\hyphenation{Ho-we-ver}
\hyphenation{de-via-tions}
\hyphenation{bio-lo-gi-cal}
\hyphenation{or-ga-nisms}

\section{History of Gompertz Equation}

In 1724 Moivre presented his hypothesis of uniform decrement, summarized in the expression $y(x)=K(w-x)$, where $y(x)$ represents the surviving
persons with age $x$, $K$ is the slope or velocity with which the population diminishes in the mortality table, and $w$ is the maximum survival
age for the population. The Moivre straight line was recommended for an age range between 12 and 86, in which it adjusted better. This linear
hypothesis was exceeded by Benjamin Gompertz, who believed in the existence of two general causes of mortality: chance and the increasing inability
of men to avoid death. Gompertz took into account only the biological causes, and his hypothesis was based on the following
idea: ``Men resistance to death diminish with time in a proportional rate'' \cite{Mina}.\\[1.5mm]
%
\indent
Benjamin Gompertz was a British mathematician interested, besides other subjects as astronomy, in the problem of life insurances and mortality
rates in the nineteenth century. He worked with death and population records of people in England, Sweden and France between ages 20 and 60 and
noted that the arithmetic increases in age were consistently accompanied by geometric increases in mortality, and that this law of geometrical
progression appeared in large portions of the different tables of mortality. Nowadays, the simple formula describing the exponential rise in death
rates between sexual maturity and extreme old age, $\gamma(t)=e^{\gamma t} $ is better known as Gompertz equation. In his first paper about this
subject published in 1820 \cite{Gompertz1820}, Gompertz identified this peculiar pattern among different european populations for a limited
portion of the age range. For his second paper, Gompertz used equal intervals of longer periods of time than in his previous work and found,
for example, that the differences in the natural logarithm between successive 10 year age intervals between ages 15 and 55 in a mortality table
for Deparceaux, France, were all nearly identical. Gompertz believed he had discovered a general law of mortality after observing similar patterns
of geometrical progression in other tables of mortality, and published it in 1825 in the Philosophical Transactions of the Royal Society, in a paper
whose title was ``On the Nature of the Function Expressive of the Law of Human Mortality'' \cite{Gompertz1825}. In his third paper he improved his
original notation and finally presented the last one in 1860, published after his death, where he noted that in his primary equation for geometric
progression, the parameters were supposed to represent constant quantities for a very long term of years \cite{Gompertz1872}. \\[1.5mm]
%
\indent
From 1825 to 1862 Gompertz was involved on the subject of what was called \emph{vital statistics} in an effort to understand why there were
consistent age patterns of death among people. Gompertz assumed that human beings have certain powers of integration and that those powers
could be divided into a principal or fundamental part and an auxiliary part responsible for the maintenance of the principal power of integration.
This auxilar force is some kind of recuperative force, a power to oppose destruction that the organisms lose in equal proportions in equal small
intervals of time. Gompertz also believed on the presence of powers destroying this auxiliary force and multiplied this hypothetical force against
life by the population alive to estimate the number of deaths in the age interval. Gompertz realized that if the force to destroy life operated
equally on everyone, then all individuals should have the same length of life, something he knew could not be true. As a possible explanation,
Gompertz emphasized the importance of chance in the timing with which death occurs. At that time the concept of genetic heterogeneity was not known,
instead, Gompertz invoked chance to explain why members of a presumed homogeneous cohort die at different times \cite{Carnes}. \\[1.5mm]
%
\indent
After Gompertz death, the subject remained mostly unknown in the scientific community. In 1860, W. M. Makeham improved Gompertz law of mortality
incorporating a term due to chance in the equation. He noted that the logarithms of the probabilities of living from Gompertz's formula increased at
a faster pace at higher age than at younger ages, so he developed a theory of partial forces of mortality that intended to explain this. Makeham
linked the diseases associated with the diminution of the vital power to specific organ systems -the lungs, heart, kidneys, stomach and liver, and
brain. These diseases represented a significant portion of total mortality at that time and worked well in solving the observed problem of greater
increased forces of mortality at older ages than at younger ages. His formula accurately portrayed the mortality experience of various human
populations between ages 10 and 95 \cite{Makeham}. \\[1.5mm]
%\begin{figure}
%\begin{center}
%\resizebox{65mm}{!}{\includegraphics{Gpzima.ps}}
%\caption{Benjamin Gompertz (1779-1865)}
%\end{center}
%\end{figure} \\[1.5mm]
%
\indent
Gompertz and Makeham recognized that the original Gompertz equation did not apply to the entire age range, the formula was intended to apply only
between the ages of 20 and 60. In fact, Gompertz suggested in his last paper that there are four distinct periods in the life span between which
separate laws of mortality apply: birth to 12 months, 12 months to 20 years, 20 years to 60 years, and 60 years to 100 years. Even within this range
he recognized that his formula worked best ``provided the intervals be not greater than certain limits.'' The applicability of the Gompertz function
to only a specified range within the life span have been recognized by many researchers but still nowadays some researchers reject the entire
Gompertz paradigm after finding that it does not apply to older ages for some organisms \cite{Carnes}. \\[1.5mm]
%
\indent
Scientists started searching biological explanations for Gompertz's law of mortality until the first years of the twentieth century, motivated in
part by the fact that increases in mortality among nonhuman species also followed Gompertz's law for a large portion of their life span. Differences
among species were assumed to be just a matter of scale. \\[1.5mm]
%
\indent
Brownlee (1919) suggested that mortality due to senescent causes should be expressed first at about age 12, become the dominant force of total
mortality by age 30, and advance at an exponential rate from ages 12 to 85. He also recognized that a law of mortality was likely to be obscured
by nonsenescent mortality. Brownlee identified a formula that accurately describes the rate of decay of substances subject to the action of organic
ferments (i.e., bacteria exposed to a disinfecting solution) which he believed produced a time dependent decay analogous to the loss of vital power.
He found that his formula corresponded to Makeham's adjustment of Gompertz's equation, leading him to the conclusion that life depends on the energy
of certain substances in the body, an energy which is gradually being destroyed throughout life \cite{Brownlee}. \\[1.5mm]
%
\indent
Wright (1926) \cite{Wrigth} appears to have first suggested the use of the Gompertz curve for biological growth. Following Wright, Davidson (1928)
used the Gompertz curve to represent the growth in body weight of cattle \cite{Davidson}. Weymouth, McMillin and Rich (1931) used the Gompertz
curve to represent the growth in shell size of the razor clam \cite{Weymouth}. They stated that the curve also gives good fits for the guinea pig
and the rat. It must be noted that they have found necessary in their most extensive series, the use of two different curves to graduate the first
and second halves of their data. Weymouth and Thompson (1931) also applied the Gompertz curve to the growth of the Pacific cockle \cite{Thompson}.
Since then, a number of authors fitted Gompertz formula to growth data for animals and organisms with remarkable success. \\[1.5mm]
%
\indent
Already in 1934, Casey fitted the Gompertz model to tumour growth data and was followed by numerous authors \cite{Casey}. The general conclusion
has been that the Gompertz law very well describes tumor growth, but a biological explanation for this success has not been found. \\[1.5mm]
%
\indent
The first person who attempted to perform an interspecies comparison of mortality, in this case, the mortality schedules of {\it Drosophila}
and humans, was Raymond Pearl. Pearl (1921) plotted the survival curves of US males in 1910 on a scale with those of the
longwinged male {\it Drosophila} \cite{Pearl1}. Although Pearl acknowledged the arbitrary nature of this comparison, particularly in the choice
of the beginning age interval for both species, he demonstrated a remarkable similarity in the curves. In his second study (1922), Pearl
refined his interspecies approach and found that the form of the  distributions was fundamentally the same \cite{Pearl2}. In addition, he found
that humans had a higher life expectancy at every age relative to the {\it Drosophila}, a discovery that he attributed to humans' control over
their environment. Pearl was the first to manipulate experimentally the living conditions of his study populations to test the importance of
accidental deaths on the survival curves. He was convinced that his research would reveal a ``fundamental biological law'' of mortality for more
than one species, but after two decades of research using this scaling approach on an expanded repertoire of species, Pearl and Minor \cite{Pearlm}
emphatically declared that a universal law of mortality did not exist. Pearl and Minor identified what Makeham had identified 68 years before as the
main problem -the inability to partition total mortality into its intrinsic and extrinsic causes of death.\\[1.5mm]
%\begin{figure}
%\begin{center}
%\resizebox{50mm}{!}{\includegraphics{pearl.ps}}
%\caption{Raymond Pearl (1879-1940)}
%\end{center}
%\end{figure} \\[1.5mm]
%
\indent
In the 50's, researchers turned to the use of radiation, which they thought was a method to accelerate senescence, for understanding aging and
making interspecies extrapolation of mortality risks. George Sacher (1950), a pioneer in this field, assumed that the effects of radiation combined
additively with natural aging, without introducing new pathology \cite{Sacher50}. Under this assumption, the Sacher model accounted for natural
aging by the inclusion of a simple linear time dependent term to the integral lethality function for radiation injury. He observed that at low
daily dose rates, the reciprocal difference in mean survival times for a control and for an irradiated population was proportional to the
intensity of exposure. In 1952 Austin Brues and George Sacher envisioned injury as a process that disrupts the normal physiological oscillations
about a mean homeostatic state within an organism, and that there were lethal injuries that an organism could not tolerate. Brues and Sacher
noted that this biological model of injury and failure lead directly to the formulation Gompertz derived to describe his law of human
mortality \cite{Brues}. Using mean survival times, Sacher estimated cumulant lethality functions to compare empirically the similarities and
differences in species' responses to radiation injury within phases of the injury process. Sacher and Trucco, however, noted that they had
insufficient knowledge about the fluctuation process in real systems and that the very fact of performing an observation introduced a disturbance
in the study \cite{Trucco}. \\[1.5mm]
%
\indent
Like Brody before him, Failla (1958) defined \emph{vitality} as the reciprocal of the age specific mortality rate \cite{Failla58}. After
expressing the Gompertz function in terms of vitality, he suggested that the resulting equation described the loss of vitality from a one hit
random process acting on the cell population. Failla concluded that the vitality curve must describe a deterioration in the function of cells
with age. He attributed the deterioration of function to somatic mutations, and interpreted the Gompertz aging parameter (derived from mortality
data) as an estimate of the spontaneous somatic gene mutation rate per cell per year. With some assumptions about generation length and the number of
genes in diploid cells, Failla (1960) calculations suggested that the mutation rate per generation was similar across
species \cite{Failla60}. This would imply that the somatic mutation rate per unit time is higher in short-lived animals than in animals
with longer life span. \\[1.5mm]
%
\indent
Szilard (1959) also developed a theory on the nature of the aging process based on the concept of accumulated somatic damage  \cite{Szilard}.
Inherited mutations in somatic genes whose function is critical late in the life span was viewed as the major explanation for the different lengths
of human beings' life. Like Sacher's lethal bound, Szilard envisioned death occurring when the fraction of somatic cells unaffected by mutation
reached a critical threshold. He suggested that the magnitude of life shortening following exposure to radiation should be inversely related to
the square root of the number of chromosomes of a species. As such, mice and humans should experience a similar radiation-induced life shortening
when expressed as a fraction of the life span. \\[1.5mm]
%
\indent
The quantitative as well as the biological importance of the Gompertz distribution was further enhanced by the work of Bernard Strehler and Albert
Mildvan (1960) \cite{Mildvan}, these investigators presented a Gompertz-based theory of mortality and aging that was based on disruptions of
the homeostatic state of an organism. Their approach differed from that of Sacher in the functional form of the equations used to describe the
disturbances of the `` energetic environment'' of an organism challenged by stress. Strehler also made several important observations of the
biological effects of radiation compared to the effects of aging. He noted that (1) aging effects are typically associated with post-mitotic cell
whereas radiation primarily affects dividing cells; (2) radiation damage is primarily genetic whereas the effects of aging appear to be more broad
spectrum; (3) some species (e.g., Drosophila) do not exhibit life shortening even after large doses of radiation; and (4) the dose required to
double the mortality rate (i.e., Gompertz slope) produces a much larger increase in the mutation rate. Based on this observations, Strehler
rejected the notion that radiation acts through a general acceleration of the normal aging process. \\[1.5mm]
%
\indent
Studies of radiation effects continued to make extensive use of the Gompertz distribution throughout the 1960's. Like Greenwood (1928) before
him \cite{Greenwood}, Grahn (1970) proposed to use the ratio of Gompertz slopes to adjust for life span differences when making mortality
comparison between species \cite{Grahn}. Grahn successfully used this scaling approach to predict reductions in human life expectancy
following radiation exposure from doses response relationships observed in mice. \\[1.5mm]
%
\indent
It seems that within the field of radiation, extrapolation between species had some success, but this differs from Pearl's conclusion that a
fundamental law of mortality applying to various species does not exist.  The reason lies on the environmental conditions of the animals being
compared, because Pearl's studies were based on the comparison with species that experienced high levels of exogenous mortality, and the laboratory
animals used in radiation studies came from controlled environments without predation and where infectious diseases were minimized. These
environmental conditions are far more similar to the sheltered environment and medical attention received by humans, leading to a better
comparison between species \cite{Carnes}. \\[1.5mm]
%
\indent
The modern development of biodemography originated with a series of articles published by Weiss and colleagues \cite{Weiss}. Weiss (1990)
recognized that the field of genetic epidemiology could provide insights into the biological constraints influencing the shape of the mortality
function in populations. Weiss's merging of the fields of demography and genetics and his subsequent elaboration using principles of
evolutionary biology served as a launching point for the latest developments in the field of biodemography. \\[1.5mm]
%
\indent
For most species survival beyond the age of reproduction is an extremely rare event with most deaths for a cohort occurring just after birth.
At these ages the vast majority of deaths result from forces of mortality that are unrelated with senescence (e.g., predation or diseases).
In this hostile environments, early reproduction has become an essential element in species' reproductive strategies (\cite{Stearns92}).
Consistent patterns of growth and development observed within species suggest that the reproductive biology of organisms alive today
represents a genetic legacy of responses to environmental conditions that prevailed during early evolutionary history of each species.
The modern evolutionary theory of senescence is based on the premise that selection is effective in altering gene frequencies until the time
before the end of the reproductive period. When the normally high force of external mortality is controlled and survival beyond the end of
reproductive period becomes a common occurrence, senescence and senescent-related diseases and disorders have the opportunity to be expressed.
Because there are common forces (i.e., extrinsic mortality) responsible for molding species'reproductive strategies, a common pattern of intrinsic
mortality, an evolutionary imprint, may become visible when species are compared on a biologically comparable time scale.
Carnes et al. \cite{Carnes2} have argued that the timing of genetically determined processes such as growth and development are driven by a
reproductive biology, molded by the necessity of early reproduction, which in turn is driven by the normally high external force of mortality.
If individual senescence is an inadvertent consequence of these developmental processes as predicted from the evolutionary theory of senescence,
then age patterns of intrinsic mortality in a population should also be calibrated to some element(s) of a species's reproductive biology.
These ideas have been introduced in various computational models. \\[1.5mm]
%
\indent
Recent mortality schedules reveal a more \emph{pure} biological influence because the external causes of death have been dramatically reduced by
medical and technological advances and almost everyone now lives to his biological potential. At the same time, a greater understanding of biological
processes has also allowed the modification of intrinsic mortality (e.g. medicine, treatments and operations) altering the survival trajectories of
individuals whose intrinsic diseases have already been expressed. From this perspective, the biological life span of a specie is one based on a
mortality schedule that would prevail in the absence of survival time manufactured by medical or pharmaceutical intervention of any kind - a view
consistent with that of Raymond Pearl. When enough members of a  population benefit from these medical interventions, it is possible that the life
span of the population will exceed its biologically based limits. All past research on mortality suggests that Gompertz was right all along: there
are biological reasons for why death occurs when it does, and a law of mortality for many species may very well exists. Which is the limit imposed
by this law of mortality for humans, and the degree to which these limits can be manipulated is still subject of great
interest \cite{Carnes}. \\[1.5mm]
%
\indent
The Gompertz equation was developed exclusively for human beings both as an empirical tool to describe the age pattern of death from all causes
during a limited time frame, and as representing a law of mortality that arises from inherent biological processes. Gompertz never imagined that
his equation would become a tool used in the analysis not only of failure time of organisms but also of failure time of mechanical devices and in
the description of biological and tumour growth.

\section{Tumour Growth Equations}

A mathematical model of tumour growth is a mathematical expression of the dependence of tumour size in time. The common feature is that growth
follows a sigmoid curve with three distinct phases: the initial exponential phase, the linear phase and the plateau. The most widely used framework
is consider tumour growth as a dynamical system described by ordinary differential equations, although some growth models are formulated successfully also by partial dif\mbox{}ferential equations. \\[1.5mm]
%
\indent The simple tumour growth model is described by a single,
first order, autonomous differential equation:

\begin{equation} \label{eq:gene}
y(t)=f(y) \qquad y(0)=y_0 >0,
\end{equation}
where $y(t) >0$ is tumour size at time $t$ and $f(y)$ is a function describing the growth rate. The solution of \eqref{eq:gene} has the remarkably
property of a monotonic ascending function of time when $f(y_0) > 0$,  or a monotonic descending function of time when $f(y_0) <0$. In the case of an
ascending function, this implies that the stationary (critical) point corresponds to the maximum possible tumor size, $y_m$,
achieved for $t \rightarrow \infty$. Similarly, in the case of a descending function, the stationary point achieved
for $t \rightarrow \infty$ is $y_s \ge 0$. The model given by Eq. \eqref{eq:gene} describes continuous tumour growth which asymptotically
approaches the finite value $y_m$ or infinity (that corresponds to the unattainable unrestricted growth). On the other
hand, \eqref{eq:gene} can describe continuous tumour regression from size $y=y_0$ to extinction ($y=0$) at some finite time or
when $t \rightarrow \infty$. However, the solution of \eqref{eq:gene} can not describe oscillatory tumour growth with regressions and
relapses. The solution $y(t)$ represents a sigmoidal ascending curve characteristic of tumour growth if a unique point of inflection
exists. This condition can be achieved for some simple functions $f(y)$. It is conceivable that functions $f(y)$ exist which yield
solutions with multiple inflection points resulting in ``multisigmoidal'' curves. Such curves would describe tumor growth with recurrent
stagnation phases \cite{Bajzer}. \\[1.5mm]
%
\indent More complex models of tumour growth kinetics are described
by systems of ordinary autonomous first-order differential
equations:

\begin{equation} \label{eq:syst}
\left\{ \begin{array}{rcl}
 \frac{dy}{dt}&=&f(y,x_1,\ldots,x_n),\\
 \frac{dx_i}{dt}&=& f_i(y,x_1,\ldots,x_n),
\end{array} \right.
\end{equation}
for $i=1,\ldots,n$ and with initial conditions $y(0)=y_0 > 0$, $x_i(0)=x_0$. Here $x_i,\ldots,x_n$ are variables describing various factors
responsible for tumour growth (e.g., levels of available nutrients, growth factor activity, size of quiescent cell population, etc.).
The functions $f$ and $f_i$ and the variables $x_i$ are chosen to represent growth mechanisms of particular interest. Unlike the simple model
given by  Eq. (\ref{eq:gene}), the system of two differential equations ($n=1$ in Eq. \eqref{eq:syst}) can describe smooth oscillatory
tumor growth \cite{Bajzer}. \\[1.5mm]
%
\indent
There is no further advance without specifying model functions $f(y)$ that represent tumor growth mechanisms. The first approach is to consider
the classical chemical kinetics paradigm, based on mass conservation. For tumour growth this paradigm can be expressed in its simplest form by:

\begin{equation} \label{eq:mass}
y(t + \triangle t) = y(t) + G(y(t)) \triangle t - D(y(t)) \triangle t.
\end{equation}
The tumor size (mass) at time $t + \triangle t$ is equal to the size
at time $t$ enlarged by $G(y(t)) \triangle t$ (generation of mass)
during the small time interval $\triangle t$, and diminished by
$D(y(t)) \triangle t$ (degradation of mass) during the same time
interval. The functions $G(y)>0$ and $D(y)>0$ are the growth and
degradation rates respectively, assumed to depend on tumor size
only. Within the limit of $t \rightarrow 0$, \eqref{eq:mass} becomes
a differential equation:

\begin{equation}\label{eq:massderi}
\frac{dy}{dt}=G(y)-D(y), \qquad y(0)=y_0 > 0.
\end{equation}
Necessary conditions for the establishment of a sigmoidal (ascending) growth curve includes:\\

\begin{itemize}
\item $G(y_0)>D(y_0)$;
\item Only one solution $y_m>y_0$ of $G(y)=D(y)$ exists as does only one solution $y_i>0$ of $\frac{dG(y)}{dy}=\frac{dD(y)}{dy}$, and
\item $y_i<y_m$.
\end{itemize}
In the latter case, $y_m$ is the maximal tumor size achieved asymptotically and $y_i$ is the tumor size at the inflection point. The stated
conditions can be met easily if both $G(y)$ and $D(y)$ are monotonic ascending functions. In a typical kinetics paradigm, these functions are given
by the power function, $ky^{n}$, where $k$ is the rate constant and $n$ is the order of the process. \\[1.5mm]
%
\indent
The second approach takes a fundamental idea:  tumor growth results from exponential cell proliferation (often called ``Malthusian growth'')
described by:

\begin{equation} \label{eq:malt}
\frac{dy}{dt}=\alpha y, \qquad \alpha > 0.
\end{equation}
This equation describes unrestricted growth leading to infinite
tumor size, a notion not supported by observation. Initially tumor
growth behaves approximately according to \eqref{eq:malt}, but
eventually it becomes stagnant due to restrictions within the tumor
itself and those imposed by the environment. Thus, exponential
growth must be modified to include terms that restrict growth. This
can be achieved by multiplying $y$ on the right-hand side of
\eqref{eq:malt} with a function $F(y) >0$ satisfying $\lim_{y
\rightarrow y_m} F(y) = 0$. The corresponding differential equation
is:

\begin{equation} \label{eq:maltm}
\frac{dy}{dt}=\alpha y F(y).
\end{equation}
Biologically, the function $F(y)$ can be interpreted as a growth function, i.e. as the ratio of proliferating cells in tumour versus total cell
population, or more generally, the ratio of growing tumour mass versus total tumour mass. The consequence of this interpretation requires
that $F(y) \le 1$ and that parameter $\alpha$ be interpreted as the growth rate constant for the hypothetical unrestricted growth. \\[1.5mm]
%
\indent
The maximal tumor size, $y_m$, predicted by the model is often designated as {\it carrying capacity}, $S>0$, of the environment for tumors in
vitro or of the host for tumors in vivo. It is useful to introduce $S$ explicitly into the growth fraction model:

\begin{equation} \label{eq:maltm1}
\frac{dy}{dt}=\alpha y g \Bigl( \frac{y}{S} \Bigl), \qquad y(0)=y_0 >0.
\end{equation}
%A tumor can reach the carrying capacity only asymptotically implying

%\begin{equation} \label{eq:cc}
%\lim_{t \rightarrow \infty} y(t)=K, \qquad g(1)=0.
%\end{equation}

%Furthermore, the solution of \eqref{eq:maltm} will represent a sigmoidal %curve if there is a unique solution $y_i<K$ of the equation:

%\begin{equation} \label{eq:maltsig}
% Kg \Bigl( \frac{y}{K} \Bigl) + y\frac{d}{dy}g \Bigl( \frac{y}{K} \Bigl)=0.
%\end{equation}

%Mathematically, the simplest realization of the function $g$ (with no free %model parameters) is a linear function: $g(z)=1-z$. Such a selection for %the growth fraction leads to the logistic model, much used in population %dynamics.\\
Mathematically, both considered approaches [yielding Eq.
\eqref{eq:massderi} or Eq. \eqref{eq:maltm1}] are equivalent and one
can easily transform one equation into the other. However, on the
vantage point of modeling and interpretation, the two approaches are
quite different. The same differential equation can yield an
intuitively acceptable interpretation in one approach, while it can
lack a transparent interpretation in the other. The paradigms of
mass conservation and growth fraction can obviously be used in
development of more elaborated models yielding systems of equations
Eq. \eqref{eq:syst} \cite{Bajzer}.

\subsection{Exponential Growth}

If the number of cells in a tumour at time $t$ is denoted by $y(t)$,
then, at time $t + \Delta t$, the number of cells would be expressed
as $y(t + \Delta t)$. The number of cells added to the tumour in the
time interval $\Delta t$ can be found subtracting $y(t + \Delta t) -
y(t)$, but this number is proportional to the duration of the time
interval (i.e. more cells arrive in a long interval than in a short
one) so:

\begin{equation}\label{eq:change}
\begin{array}{rcl}
y(t + \Delta t) - y(t) & =&  N \Delta t,\\
\frac{y(t + \Delta t) - y(t)}{\Delta t}  &=&  N.
\end{array}
\end{equation}

Suppose that the increase in number of the cell population is due entirely to cells being born. As time progresses the division or birth rate
may be altered so that more or less divisions occur, so the number of cells born in the interval $\Delta t$ may vary with time. Moreover, if there
are more cells at time $t$, more divisions are likely to occur and $N$ will also depend on $y(t)$. Letting $\Delta t \rightarrow 0$, the left-hand
side of Eq. \eqref{eq:change} becomes the derivative of $y$ with respect to $t$, and we have:

\begin{equation}\label{eq:deriva1}
\frac{dy(t)}{dt}=N\{t,y(t)\},
\end{equation}
where we show explicitly the quantities on which $N$ depends. The expression $(1/y)(dy/dt)$ is known as the {\bf specific growth rate}. Therefore,
another way of describing Eq. \eqref{eq:deriva1} is to say that the specific growth rate is $N(t,y)/y$. \\[1.5mm]
%
\indent
It is plausible to assume that, in a short time interval, there will be about twice as many births as in a time interval of half its length.
Thus, one could expect that the number of births would be proportional to $y(t)\Delta t$ when $\Delta t$ is small. If the birth rate does not
change in the time interval, $\Delta t$ can be expressed as $\alpha y(t) \Delta t$ with $\alpha$ a suitable constant.
Then Eq. \eqref{eq:deriva1} becomes:

\begin{equation}\label{eq:derino}
\frac{dy(t)}{dt}=\alpha y(t),
\end{equation}
which states that the specific growth rate is $\alpha$, the same for
all times and all sizes of tumour. This equation has the same form
of the expression found in Eq. \eqref{eq:malt} and its solution can
be realized by the following procedure:

\begin{equation}\label{eq:derinosol}
\begin{array}{rcl}
\alpha \int_{0}^{t}dt & = &\int_{y(0)}^{y(t)} \frac{dy}{y},\\
\alpha t & = &ln\{y(t)/y(0)\},\\
%e^{N_0 t} & = &\frac{y(t)}{y(0)}
\end{array}
\end{equation}

leading to:

\begin{equation}\label{eq:derisolf}
y(t)=y_0 e^{\alpha t},
\end{equation}
where $y_0$ is any constant that can be fixed by putting $t=0$ in Eq. \eqref{eq:derisolf}, and evidently is the size of the tumour at $t=0$. \\\\
\begin{figure}[h]
\begin{center}
\begin{minipage}[c]{10.5cm}
\includegraphics[width=0.9\textwidth]{expoa.eps}
\end{minipage}
\caption{Exponential growth, with $y_0=1$, $\alpha =1$. See Eq. \eqref{eq:derisolf}}
\label{fig:exponential}
\end{center}
\end{figure}\\[1.5mm]
%
\indent
The behaviour of a tumour, or a population, as time increases according to \eqref{eq:derisolf} is displayed in figure (\ref{fig:exponential}).
The size grows steadily, and the increase becomes dramatic as time goes on. Of course, in any real situation, there will be a limit to the growth
because of a shortage of essential supplies or insufficient food. Nevertheless, many organisms exhibit exponential growth in their initial
stages \cite{Jones}.\\[1.5mm]
%
\indent
%It is always easy to check where a population is growing exponentially by %plotting $\ln y$ against time; a straight line %should be obtained. The %slope of the line is the specif\mbox{}ic growth rate $N_0$ as is clear %from \eqref{eq:derinosol}.\\
%\begin{figure}[htp]   usar package graphicx!
%\begin{center}
%\includegraphics[height=100mm,width=60mm,angle=-90]{expon.%eps}
%\caption{Graph of exponential growth,with $p_0=1$, %$N_0=1$.}
%\end{center}
%\end{figure}
Notice that Eq. \eqref{eq:derino} has been derived on the assumption that only births can occur. In the event that there are deaths but no births
the same equation can be reached.  However, $\alpha$ is now a negative number since the population or cell number decreases in the time
interval $\Delta t$. It follows from \eqref{eq:derisolf} that the population decays exponentially with time from its
size at $t=0$.\\[1.5mm]
%
\indent
More facets of the population problem can be incorporated in this equation. For instance, we may postulate that the number of deaths in
the short time interval $\Delta t$ is $\beta y(t) \Delta t$. Similarly, individuals may enter the given area from outside,
say $I(t) \Delta t$ immigrants in the interval $\Delta t$. Likewise, some may depart from the area giving rise to $E(t) \Delta t$ emigrants.
We can model this population facets via the following equation:

\begin{equation}\label{eq:Verh}
y(t+\Delta t)-y(t)= \alpha y(t)\Delta t - \beta y(t)\Delta t + I(t)\Delta t-E(t)\Delta t,
\end{equation}
leading to:

\begin{equation}\label{eq:Verhulst}
\frac{dy(t)}{dt}= \bigl( \alpha-\beta \bigl)y(t) +I(t)-E(t),
\end{equation}
when $\Delta t \rightarrow 0$. More generally, $I$ and $E$ could be
made to depend on $y$ so that Eq. \eqref{eq:Verhulst} (often called
{\bf Verhulst´s differential equation}) can be difficult to solve.
Notwithstanding, it is transparent that, if we hope to predict the
size of a population at a given time, to find the solution of a
differential equation will be an essential requirement \cite{Jones}.

\subsection{Logistic Growth}

A characteristic that must be taken into account is that the
multiplication in cell numbers is restricted by crowding effects.
Biochemically, these may be due to lack of nutrients, shortage of
oxygen, change in pH or the production of inhibitors, for example.
Whatever the cause, the cells are interacting between them. Since
each cell can interact with $y$ others, there are $y^{2}$
possibilities in total. This suggests that, in Eq.
\eqref{eq:deriva1}, we should put:

\begin{equation}\label{eq:cell}
N\{t,y(t)\}=\alpha y(t)-\beta y(t)^{2},
\end{equation}
where $\alpha$ and $\beta$ are positive constants. The term involving $\alpha$ is the same as before and takes into account the increase
due to division. The term containing $\beta$ represents the inhibition on growth causes by crowding. With the substitution of Eq. \eqref{eq:cell}
toward  Eq. \eqref{eq:deriva1} we have:

\begin{equation}\label{eq:logistic}
\frac{dy}{dt}=\alpha y - \beta y^{2},
\end{equation}
which is called the {\bf differential equation of logistics.} In the growth fraction paradigm Eq. \eqref{eq:maltm1}, the equation equivalent
to Eq. \eqref{eq:logistic} is:

\begin{equation}\label{eq:logistic2}
\frac{dy}{dt}= \alpha y (1 - y/S),
\end{equation}
where $S=\alpha / \beta$.\\[1.5mm]
%
\indent
If we integrate Eq. \eqref{eq:logistic} from $0$ to $t$, we obtain:

\begin{equation}\label{eq:logsol}
\begin{array}{rcl}
\int_{0}^{t}dt & = &\int_{y(0)}^{y(t)}\frac{dy}{\alpha y-\beta y^{2}},\\
t & =  & \frac{1}{\alpha} \int_{y(0)}^{y(t)} \Bigl ( \frac{1}{y} - \frac{\beta}{\beta y-\alpha} \Bigl )dy,\\
 & =  & \frac{1}{\alpha} ln \Bigl ( \frac{y}{\beta y-\alpha} \Bigl) \vert_{y(0)}^{y(t)},\\
 & = & \frac{1}{\alpha} ln \Bigl( \frac{y(t)\{\beta y(0)-\alpha\}}{y(0)\{\beta y(t)-\alpha\}} \Bigl) .
\end{array}
\end{equation}
Hence, solving for $y(t)$, we have:

\begin{equation}\label{eq:logsol1}
\begin{array}{rcl}
y(t) \{ \beta y(0)-\alpha \} = \{ \beta y(t)-\alpha \} y(0) e^{\alpha t}\\
y(t)=\frac{\alpha y(0)}{\beta y(0)+ \{ \alpha -\beta y(0) \} e^{-\alpha t}},
\end{array}
\end{equation}
which is known as the {\bf logistic law of growth}. In terms of the carrying capacity $S = \alpha / \beta$, Eq. \eqref{eq:logsol1} takes the
next form:

\begin{equation}\label{eq:logsol2}
\begin{array}{rcl}
y(t)=\frac{S y(0)}{y(0)+ \{ S - y(0) \} e^{-\alpha t}}.
\end{array}
\end{equation}

The logistic curve is used to model a great variety of physical situations in which growth of a quantity is ``self-limited'', that is, the growth
rate of the quantity depends on the size of the quantity in such a way that if the quantity grows beyond a certain level, the growth rate decreases.
The logistic model nicely describes the behaviour of certain types of growth in business, economics, populations and sales forecasts \cite{Jones}.\\\\
\begin{figure}[h]
\begin{center}
\begin{minipage}[c]{10.5cm}
\includegraphics[width=0.9\textwidth]{logistica.eps}
\end{minipage}
\caption{Logistic curve with $\alpha=3$, $\beta=1$, $y(0)=1$.}
\label{fig:logistic}
\end{center}
\end{figure}\\[1.5mm]
%
\indent The curve of logistic growth is shown in figure
(\ref{fig:logistic}), assuming that $\alpha > \beta y(0)$. The curve
rises steadily from the value $y(0)$ at $t=0$ to an eventual value
of $\alpha / \beta$, there being neither maxima nor minima in the
curve. There is, however, a point of inflexion where the curve
crosses its tangent at $t=t_0$ where:
\begin{equation}\label{eq:poinf}
t_{0}=\frac{1}{\alpha}ln \Bigl(\frac{\alpha}{\beta y(0)} - 1 \Bigl),
\end{equation}

and $y(t_0)=\alpha / 2 \beta$.\\

Notice that the final value $\alpha / \beta$ of $y$ does not involve $y(0)$, so that, no matter what the initial size of the population,
its final size is always the same and does not depend on the starting size of the population.\\[1.5mm]
%
\indent
In 1838, Verhulst proposed this model as a description of population growth. The model had been virtually forgotten
until Pearl ``rediscovered'' it years later. Since then it has been often used as a point of departure for more advance population models.
In 1945, Rashevsky, one of the founders of modern mathematical biology, arrived to the logistic model by considering tumor growth.
Interestingly, the logistic model was used for fitting to tumor growth data much less frequently than the Gompertz model. On the other hand, the
logistic model has been used in kinetics models describing immune response to tumor, where it has served as a mathematically simple description of
immunologically unaffected tumor growth. Similarly, the logistic model has been used in models for chemotherapy
optimization \cite{Bajzer}.\\[1.5mm]
%
\indent
It is important to remember that the logistic law assumes that all cells divide at the same rate, and this is not always true. There are
types in which some cells divide faster than others. Whether the logistic law can be applied still depends upon the differences between the
various rates of division present. If the rates are not too far apart it is probably feasible to take $\alpha$ as their average. For greater
deviations may be necessary to adopt a model in which the statistics of the number of cells of a given age and type at a given time play a
part \cite{Jones}.\\[1.5mm]
%
\indent
The immediate generalization of the logistic model Eq. \eqref{eq:logistic} is:

\begin{equation} \label{eq:logral}
\frac{dy}{dt}= \alpha y - \beta y^{\nu}, \qquad \nu > 1,
\end{equation}

with solution

\begin{equation} \label{eq:logrsol}
y=\Bigl[ k-\Bigl( k-y_0^{1-\nu} \Bigl) e^{\alpha(1-\nu)t} \Bigl] ^{\frac{1}{(1-\nu)}}, \qquad k=\frac{\alpha}{\beta}.
\end{equation}

Function \eqref{eq:logrsol} is often designated as the Richard
function. The solution of Eq. \eqref{eq:logral} has been thoroughly
discussed by Fletcher. Interestingly, when this model was fitted to
tumor growth data with $y_0$, $\alpha$, $\beta$, and $\nu$ as free
parameters, in most cases it was found that $\nu \approx 1$.
Clearly, $\nu$ cannot be exactly 1, because then \eqref{eq:logral}
would describe unrestricted exponential growth. However, if
\eqref{eq:logral} is reparametrized somewhat peculiarly as:

\begin{equation} \label{eq:logrep}
\frac{dy}{dt}= \Bigl( a+\frac{b}{\nu-1} \Bigl)y - \frac{b}{\nu-1} y^{\nu} = ay - by\frac{y^{\nu-1}-1}{\nu-1},
\end{equation}
then in the limit $\nu  \rightarrow 1$ one obtains the Gompertz
model $dy/dt =ay-by \ln y$, using the general result: $\lim_{x
\rightarrow 0} \frac{c^{x}-1}{x}= \ln c.$. The result that fitting
to data yielded $\nu \approx 1$ can be interpreted as a clear
indication that the Gompertz model is a much more adequate
description of tumor growth kinetics than is the logistic model
\cite{Bajzer}.


\subsection{Von Bertalanffy Growth}

The combination of the chemical kinetics paradigm and the principle
of allometry led von Bertalanffy to formulate the model of
organismic growth represented by the equation:

\begin{equation} \label{eq:bert}
\frac{dy}{dt}= \alpha y^{\mu} - \beta y^{\nu}, \qquad \mu >0, \qquad \nu > 0.
\end{equation}

It was shown that for any $\mu$ and $\nu$ the solution of Eq.
\eqref{eq:bert} can not be expressed in terms of elementary
functions, but in terms of the modified beta-function,

\begin{equation} \label{eq:betafun}
\beta(x,r,s)= \int_{1/2}^{x}(1-u)^{r-1}u^{s-1}\,du
\end{equation}
and its inverse.\\[1.5mm]
%
\indent The model characterized by $\mu = 2/3$ and $\nu=1$ is based
on the so called ``surface rule'', which is often named von
Bertalanffy model. The underlying notion is that the anabolic growth
rate is proportional to the surface area (expressed as $y^{2/3}$
where $y$ is interpreted as volume), and the catabolic growth rate
is proportional to the volume itself. Another especial case of Eq.
\eqref{eq:bert} is the generalized logistic model with $\mu=1$,
presented by Eq. \eqref{eq:logral}, and its counterpart with
$\nu=1$:

\begin{equation} \label{eq:espcase}
\frac{dy}{dt}= \alpha y^{\mu} - \beta y, \qquad \mu < 1.
\end{equation}
The solution of this equation is of the same form as Eq. \eqref{eq:logrsol}, because Eq. \eqref{eq:espcase} can be formally transformed
into Eq. \eqref{eq:logral} by parameter redefinition, as clearly presented by Fletcher. Obviously, model Eq. \eqref{eq:espcase} contains the
von Bertalanffy ``surface rule'' model.\\[1.5mm]
%
\indent
Returning to the general model Eq. \eqref{eq:bert}, we wish to point out its not obvious relationship to the Gompertz model. Similarly to the
generalized logistic model, Eq. \eqref{eq:bert} can be reparametrized into:

\begin{equation} \label{eq:vberpa}
\frac{dy}{dt}=ay^{\mu} -  \frac{1}{\epsilon}by^{\mu}(y^{\epsilon}-1).
\end{equation}
In the limit $\epsilon \rightarrow 0$, one then obtains the so called ``generalized Gompertz model'':

\begin{equation} \label{eq:gragom}
\frac{dy}{dt}=ay^{\mu} - by^{\mu} \ln y,
\end{equation}
which for $\mu=1$ reduces to the original Gompertz model. In
practice, this means that tumor growth data described by the
generalized von Bertalanffy model with $\mu \approx 1$, $\nu \approx
1$, are described also by the Gompertz model \cite{Bajzer}.

\subsection{Gompertz-Makeham Growth}

In the paradigm of chemical kinetics (see Eq. \eqref{eq:massderi}), the equation

\begin{equation} \label{eq:ckgo}
\frac{dy}{dt}= \alpha y - \beta y \ln y, \qquad  y(0)=y_0 >0,
\end{equation}
has the Gompertz growth formula as the unique solution. The growth rate $\alpha y$ reflects the Malthusian law with clear interpretation,
but the degradation rate lacks any such interpretation.\\[1.5mm]
%
\indent
In the growth fraction paradigm (Eq. \eqref{eq:maltm1}), the equation equivalent to Eq. \eqref{eq:ckgo} is obtained for $g(z)=-\ln z$, i.e.

\begin{equation} \label{eq:ckgogf}
 \frac{dy}{dt}=-\gamma y \ln \Bigl( \frac{y}{S} \Bigl), \qquad y(0)=y_0 > 0.
\end{equation}
Thus the growth fraction $g(z)$ is the simplest possible elementary transcendental function which obeys $g(z) \in [0,1)$ for $z \in (0,1]$
with $g(1)=0$. Besides the simplicity argument, there is not an obvious interpretation of the growth fraction function.
The solution of Eq. \eqref{eq:ckgogf} and Eq. \eqref{eq:ckgo} reads:

\begin{equation} \label{eq:cksol}
\begin{array}{rcl}
y & = & y_{0}e^{(\alpha / \beta - \ln y_{0})(1-e^{-\beta t})}\\
y & = & y_{0}e^{\ln (S/y_{0})(1-e^{-\gamma t})}\\
  & = & Se^{-\ln (S/y_{0})e^{-\gamma t}}.
\end{array}
\end{equation}

Comparison of \eqref{eq:ckgo} and \eqref{eq:ckgogf} yields interesting relations among parameters:

\begin{equation} \label{eq:compara}
\beta = \gamma, \qquad \alpha = \gamma \ln S.
\end{equation}
These relations suggest that the inherent growth rate constant $\gamma$ (the rate constant for unrestricted growth, i.e., $S \rightarrow \infty$ )
is equal to the degradation rate constant $\beta$  and yet $\gamma$ is also proportional to the Malthusian growth rate constant $\alpha$.
This indicates that the Gompertzian growth is regulated by the parameter $\gamma$ which controls both growth and degradation \cite{Bajzer}.\\[1.5mm]
%
\indent
If we start from Eq. \eqref{eq:ckgogf} and declare the growth fraction a new time dependent variable:

\begin{equation} \label{alt}
x=g(\frac{y}{S})= \ln \Bigl( \frac{S}{y} \Bigl).
\end{equation}
The solution \eqref{eq:cksol} satisfies also the system of
equations:

\begin{equation} \label{eq:systalt}
\begin{array}{l}
 \frac{dy}{dt}= \gamma xy,\\
 \frac{dx}{dt}=-\gamma x,
\end{array}
\end{equation}
with initial conditions $y(0)=y_{0}$ and $x(0)=\ln (S/y_{0})$. From
here, it is clear that the parameter $\gamma$ is at the same time
the inherent growth rate constant and the rate constant for the
temporal decrease of the growth fraction. This certainly is a
peculiarity of the Gompertz model which supports the idea that the
single parameter $\alpha$ controls an inhibitory feedback mechanism
operating in tumors. Beyond this and beyond the transparent
structure of Eq. \eqref{eq:systalt}, that has a simple
interpretation, other fundamental insights are not apparent. Another
possibility to present the Gompertz model as a system of two
differential equations is based on the introduction of the effective
growth rate $x'_{1}=\gamma x$ as a variable:

\begin{equation} \label{eq:systgra}
\left\{ \begin{array}{l}
 \frac{dy}{dt}= x_1 y,\\
 \frac{dx_1}{dt}= \gamma x_1.
\end{array} \right.
\end{equation}
This system of equations is interpreted as describing exponential growth with exponential retardation. However, this can be inferred
directly from Eq. \eqref{eq:ckgo}.

\subsection{Mathematical Properties and Comparison Between Logistic and Gompertz Growth}

It is convenient to write equation Eq. (\ref{eq:cksol}) as:

\begin{equation} \label{eq:gompm}
y=ce^{-e^{a-bx}},
\end{equation}
in which $c$ and $b$ are essentially positive quantities. From Eq. \eqref{eq:gompm} it is clear that as $x$ becomes negatively
infinity $y$ will approach zero, and as $x$ becomes positively infinity $y$ will approach $c$. Differentiating Eq. \eqref{eq:gompm} we have:

\begin{equation} \label{primder}
\frac{dy}{dx} = cbe^{a-bx}e^{-e^{a-bx}}=bye^{a-bx},
\end{equation}
and it is apparent that the slope is always positive for finite values of $x$, and approaches zero for infinite values of $x$. Differentiating again:

\begin{equation} \label{eq:segder}
\frac{d^{2}y}{dx^{2}} = b^{2}ye^{a-bx}(e^{a-bx}-1),
\end{equation}
and we obtain the point of inflection in:

\begin{equation} \label{eq:inflex}
x = \frac{a}{b} ;\qquad
y = \frac{c}{e},
\end{equation}
or approximately, when 37 \% of the final growth has been reached. Therefore, when we desire to fit growth data which show a point of inflection
in the early part of the growth cycle, we may use the Gompertz curve with the expectation that the approximation to the data will be good.
Notice Figure 1, which shows the form of the curve for the case $c=1$, $a=0$, $b=1$; there are also shown the logistic and the first derivative
of the Gompertz curve \cite{Winsor}.
\begin{figure}[h]
\begin{center}
\begin{minipage}[c]{10.5cm}
\includegraphics[width=0.9\textwidth]{compa.eps}
\end{minipage}
\caption{Gompertz curve and its first derivative, and the logistic curve,
with $c=1$, $a=0$, $b=1$.}
\label{fig:comp}
\end{center}
\end{figure}\\[1.5mm]
%
\indent
The logistic possesses the same number of constants as the Gompertz curve, but has the point of inflection mid-way between the asymptotes. It is
described by the following equation:

\begin{equation} \label{eq:logisticw}
y = \frac{c}{1+e^{a-bx}}.
\end{equation}
It has been found useful to add a constant term to the logistic, giving it a lower asymptote different from zero:

\begin{equation} \label{eq:logycte}
y = d + \frac{c}{1+e^{a-bx}}.
\end{equation}

This procedure is equally applicable to the Gompertz curve giving:

\begin{equation} \label{eq:gomycte}
y = d + ce^{-e^{a-bx}}.
\end{equation}

The Gompertz curve and the logistic possess similar properties which make them useful for the empirical representation of growth phenomena. Each
curve has three arbitrary constants, which corresponds essentially to the upper asymptote, the time origin, and the time unit or rate constant. In
each curve, the degree of skewness, as measured by the relation of the ordinate at the point of inflection to the distance between the asymptote, is
fixed \cite{Winsor}.\\[1.5mm]
%
\indent
To illustrate the mathematical properties of the Gompertz and logistic curves, the table from \cite{Winsor} has been reproduced on the
next page.\\[1.5mm]
%
\indent
The Gompertz equation is used as a predictive tool in demography \cite{MuellerN}. However, the Gompertz law of exponential increase in mortality
rates with ages is observed in many other biological species, such as rats, mice, fruit flies and flour beetles \cite{Gavrilov}, not only on
humans, and, therefore, some general theoretical explanation for this phenomenon is required. Furthermore, it often fits growth of organisms,
organs and tumours. Despite numerous attempts, no consensus has been forged about the biological foundation of the broad applicability of
the model \cite{Vuk}.\\

\begin{table}[h]
\begin{center}
\begin{tabular}{|p{3.8cm}|p{3.6cm}|p{3.2cm}|}
\hline
CURVE & GOMPERTZ & LOGISTIC \\
\hline
Equation & $y=ce^{-e^{a-bx}}$ &
 $y=\frac{1}{1+e^{a-bx}}$ \\
\hline
Number of Constants & 3 & 3\\
\hline
Asymptotes & $y=0, y=c$ & $y=0, y=c$\\
\hline
Inflection & $x=\frac{a}{b}, y=\frac{c}{b}$ & $x=\frac{a}{b}, y=\frac{c}{2}$ \\
\hline
Straight line of equation & $loglog\frac{c}{y}=a-bx$ & $log\frac{c-y}{y}=a-bx$ \\
\hline
Symmetry & Assymetrical & Symmetrical about inflection \\
\hline
Growth rate & $\frac{dy}{dx} = bye^{a-bx}=bylog\frac{c}{y}$ & $\frac{dy}{dx} = \frac{b}{c}y(c-y)$\\
\hline
Maximum growth rate & $\frac{bc}{e} $ & $\frac{bc}{4} $ \\
\hline
Relative growth rate as function of time & $\frac{1}{y}\frac{dy}{dx} = be^{a-bx} $ & $\frac{1}{y}\frac{dy}{dx} = \frac{b}{1+e^{-a+bx}} $ \\
\hline
Relative growth rate as function of size & $\frac{1}{y}\frac{dy}{dx} = b(logc-logy)$ & $\frac{1}{y}\frac{dy}{dx} = \frac{b}{c}(c-y)$ \\
\hline
\end{tabular}
\caption{Mathematical properties of Gompertz and logistic curves.}
\end{center}
\end{table}


==> capitulouno.tex <==
\chapter{Monte Carlo Simulations in Statistical Physics}
\minitoc
%\bibliographystyle{plain}
\clearpage

\hyphenation{de-ve-lop-ment}
\hyphenation{co-mmu-ni-ty}
\hyphenation{i-mme-dia-te-ly}
\hyphenation{o-pe-ra-tions}
\hyphenation{su-gges-ted}
\hyphenation{e-xam-ple}
\hyphenation{pro-blems}
\hyphenation{pu-bli-shed}
\hyphenation{wi-shing}
\hyphenation{o-pe-ra-tio-nal}
\hyphenation{e-xa-mi-ne}
\hyphenation{con-si-de-ring}
\hyphenation{e-qui-li-brium}
\hyphenation{con-fi-gu-ra-tions}


\section{Brief History of the Monte Carlo Method}

The first electronic computer, ENIAC, was developed during the World War II period by a group of scientists working at the University of
Pennsylvania in Philadelphia. They had realized that if electronic circuits could be made to count, then they could do arithmetic and hence,
solve difference equations at incredible speeds. This would lead to a scientific revolution because it would give the possibility to study problems
unsolved before due to the large amount of calculations needed. \\[1.5mm]
%
\indent
In 1946, Stanislaw Ulam, a mathematician working in Los Alamos, attended a conference about a preliminary computational model of a thermonuclear
reaction probed in ENIAC as a test for the computer. Like other scientists, he was impressed by the speed and versatility of the ENIAC.
Additionally, Ulam's extensive mathematical background made him aware that statistical sampling techniques that had fallen into disuse
because of tediousness of calculations, could be resuscitated with ENIAC. The basis of the Monte Carlo method has been proposed later by
him as a consequence of his interest in random processes. As Stan Ulam mentioned in 1983, his first thoughts and attempts to practice the Monte
Carlo method were suggested by a question that occurred to him in 1946 as he was playing solitaires. The question was what were the chances that a
Canfield solitaire laid out with 52 cards will come out succcessfully? \footnotemark. After spending a lot of time trying to estimate them
by pure combinatorial calculations, he wondered whether a more practical method might not be to lay it out say one hundred times and simply
observe and count the number of successful plays. \footnotetext[1]{Today is quite well known that the chance of winning is low: 3.3\%
(www.games.solitaire.com)} He immediately thought about how to change processes described by certain differential equations into an equivalent
form interpretable as a succession of random operations \cite{Eckhardt}. Ulam discussed his ideas with John von Neumann,
Professor of Mathematics at the Institute for Advanced Study at Princeton, who was also a consultant to Los Alamos and one of the principals
participating in the ENIAC probe conference in 1946. Von Neumann saw the importance of Ulam's approach and thought that it seemed especially
suitable for exploring the behaviour of neutron chain reactions in fission devices. In March 1947, von Neumann wrote to Robert Richtmyer,
the Leader of the Theoretical Division at Los Alamos, describing a possible statistical method to solve the problem of neutron diffusion in
fissionable material using the newly developed electronic computing techniques. It was at that time when Nicholas Metropolis suggested the
name Monte Carlo for this statistical method. It was related to the fact that Stan had an uncle who would borrow money from relatives because
he ``just had to go to Monte Carlo'' \cite{Metropolis} and also because of the similarities between the method and the games of chance abundant
in the capital of Monaco, the european center of gambling.\\[1.5mm]
%
%\begin{figure}
%\begin{center}
%\resizebox{50mm}{!}{\includegraphics{ulam.ps}}
%\caption{Stanislaw Ulam (1909-1984) \cite{fotoulam}.}
%\label{fig:ulam}
%\end{center}
%\end{figure}
%
\indent Very similar methods, not fully developed, had been used
earlier. An example is Buffon's needle problem, an experiment
performed in the
 of the eighteenth century, which represents one of the first problems in geometric probability. It consists in throwing a needle randomly on a board with parallel lines, and inferring the value of $\pi$  from the number of times the needle intersects a line \cite{Hall}; nowadays, Buffon's needle problem is practically solved by Monte Carlo integration. Descriptions of several modern Monte Carlo techniques appear in a paper by Kelvin \cite{Kelvin}, written nearly one hundred years ago, in the context of a discussion on the Boltzmann equation. In the 1940's, Enrico Fermi also used Monte Carlo in the calculation of neutron dif\mbox{}fusion, and later designed the Fermiac, a Monte Carlo mechanical device used in the calculation of criticality in nuclear reactors \cite{Anderson}. Ulam's contribution was to recognize the potential for the newly invented electronic computer to automate such sampling.\\[1.5mm]
%
\indent
The approach proposed by von Neumann in his letter was the first formulation of a Monte Carlo computation for an electronic machine.
Von Neumann considered a spherical core of fissionable material surrounded by a shell of normal material, and the idea was to trace out the development of neutrons using random digits to select the outcomes of the various interactions along the way, such as scattering, absorption and f\mbox{}ission. For example, once a neutron is selected to have an initial position with certain velocity, you have to decide the position of the f\mbox{}irst collision and the nature of the collision. If you select a f\mbox{}ission to occur, then the number of emerging neutrons must be chosen, and each of the new neutrons is followed too. On the other hand, if you decide that the outcome of the collision is scattering, the new momentum of the neutron must be determined. If the neutron crosses a material boundary, the characteristics of the new medium must be taken into account. At the end, a genealogical history of a neutron emerges. The same procedure is carried out for other neutrons until a statistically valid picture is obtained. Each neutron history is analogous to a single game of solitaire, and the use of random numbers to make the choices along the way is analogous to the random turn of the card. \\[1.5mm]
%
\indent To take decisions, the computer must have an algorithm for
generating a uniformly distributed set of random numbers and these
numbers must be transformed into the nonuniform distribution, say
$g$, desired for the property of interest. In a 1947 letter, von
Neumann discussed two techniques for using uniform distributions of
random numbers to generate $g$. The first technique, which had
already been proposed by Ulam, shown that the function $f$ needed to
achieve this transformation is just the inverse of the nonuniform
distribution function, that is, $f=g^{-1}$. For example, in the case
of neutron physics, the distribution of free paths (how far neutrons
of a given energy in a given material go before colliding with a
nucleus) decreases exponentially with distance. If $x$ is uniformly
distributed in the open interval $(0,1)$, then $f= - \ln x$ will
give us a nonuniform distribution $g$ with just those properties.
The rest of von Neumann letter describes an alternative technique
that works when it is difficult or computationally expensive to form
the inverse function, which is frequently true when the desired
function is empirical. In this approach, two uniform and independent
distributions $(x_i)$ and $(y_i)$ are used. If two numbers $x_i$ and
$y_i$ are selected randomly from the domain and range, respectively,
of the function $f$, then each such pair of numbers represents a
point in the function's coordinate plane $(x_i,y_i)$. When $y_i >
f(x_i)$ the point lies above the curve for $f(x)$, and $x_i$ is
rejected; when $y_i \leq f(x_i)$ the point lies on or below the
curve, and $x_i$ is accepted (see Fig. \ref{fig:distribution}). Thus
the fraction of accepted points is equal to the fraction of the area
below the curve. In fact, the proportion of points selected that
fall in a small interval along the $x$-axis will be proportional to
the average height of the curve in that interval, ensuring
generation of random numbers that mirror the desired distribution
\cite{Eckhardt}.
%
\begin{figure}[h]
\begin{center}
\resizebox{60mm}{!}{\includegraphics{probfunc.ps}}
\caption{Generation of random numbers that mirror a given
distribution $f(x)$ \cite{Eckhardt}.} \label{fig:distribution}
\end{center}
\end{figure}\\[1.5mm]
%
\indent
The first ambitious test of the Monte Carlo method consisted of nine problems in neutron transport, each one corresponding to various configurations
of materials, initial distributions of neutrons, and running times. These problems did not include hydrodynamic and radiative effects, but complex
geometries and realistic neutron-velocity spectra were handled easily. Neutron histories were checked with a variety of statistical analyzes and
comparisons with other approaches. Conclusions about the efficiency of the method were quite favourable and gave rise to enthusiasm among
scientists of distinct areas. At Los Alamos, the method was quickly adopted to study problems of thermonuclear and fission devices. Already in
1948, Ulam was able to report to the Atomic Energy Commission about the applicability of the method for cosmic rays and in the area of the
Hamilton Jacobi partial differential equation. Other laboratory staff members started to run Monte Carlo codes in ENIAC. Among them,
J. Calkin, C. Evans and F. Evans studied thermonuclear problems, and B. Suydam and R. Stark tested the concept of artificial viscosity for
time-dependent shocks. By midyear 1949, Ulam and Metropolis published a paper describing the Monte Carlo method and its application to
integro-differential equations \cite{MetroUlam} and the first symposium on the method was held in Los Angeles.\\[1.5mm]
%
%\begin{figure}[h]
%\begin{center}
%\resizebox{110mm}{!}{\includegraphics{neumann.ps}}
%\caption{John von Neumann (1903-1957) in front of the ENIAC \cite{fotoneumann}.}
%\label{fig:neumann}
%\end{center}
%\end{figure}\\[1.5mm]
%
\indent The construction of a new machine began later and N.
Metropolis was the leader of the group in charge of it. He called
the new machine MANIAC wishing to stop the use of acronyms for
machine names, but contrary to what he sought, it only stimulated
it. In early 1952, the MANIAC became operational at Los Alamos and
soon after, Anthony Turkevich led a study of the nuclear cascades
resulting from the collision of accelerated particles with atomic
nuclei. Another computational problem run on the MANIAC was a study
of equations of state based on the two-dimensional motion of hard
spheres. The results were published in a famous paper in 1953
\cite{MetroTeller} and describes a strategy leading to greater
computational efficiency for equilibrium systems obeying the
Boltzmann distribution function. The idea developed in that
 is that if a move of a particle in the system causes a decrease in the total energy, the new configuration should be accepted. On the other
 hand, if there is an increase in energy, the new configuration is accepted only if it passes through a game of chances biased by a
 Boltzmann factor, otherwise, the old configuration is kept.\\[1.5mm]
%
%\begin{figure}[h]
%\begin{center}
%\resizebox{50mm}{!}{\includegraphics{metropolis.ps}}
%\caption{Nicholas Metropolis (1915-1999) \cite{fotometro}.}
%\label{fig:metropolis}
%\end{center}
%\end{figure}\\[1.5mm]
%
\indent Since then, the Monte Carlo method has been proved to be a
very powerful and useful tool. For example, deterministic methods
for numerical integration of functions with many variables are very
inefficient because with every additional dimension or variable, an
exponential time increase takes place. The alternative way provided
by the Monte Carlo method is the following: the function in question
can be estimated by randomly selecting points in the many
dimensional space and taking some kind of average of the values of
the function at these points. This method will display $1/ \sqrt{N}$
convergence, i.e. quadrupling the number of sampled points will
halve the error, regardless of the number of dimensions. The use of
Monte Carlo methods to model physical problems allows us to examine
more complex systems that otherwise we are not able to handle.
Solving equations which describe the interactions between two atoms
is fairly simple but solving the same equations for hundreds or
thousands of atoms is impossible. With Monte Carlo methods, a large
system can be sampled in a number of random configurations, and
those data can be used to describe the system as a whole. There are
currently many applications of the Monte Carlo method: stellar
evolution \cite{stellar}, reactor design \cite{reactor}, cancer
therapy \cite{cancertherapy}, traffic flow \cite{vehicular}, finance
\cite{finances}, simulations of various systems of interacting
particles (e.g. ferromagnetic materials), grain growth modeling in
metallic alloys \cite{growth,Rollett}, the behaviour of
nanostructures and polymers \cite{nano}, and protein structure
predictions \cite{protein}.

\section{Basics of the Monte Carlo Method}

In statistical mechanics, the partition function $Z(H,T)$ contains all the necessary information to calculate the thermodynamic
properties of a system. The difficulty arise when the size of the system and the number of degrees of freedom for each particle is large,
something that occurs in almost all cases. Then, summing over the large number of possible states to calculate $Z(H,T)$ is extremely expensive
and almost impossible even in a computational way. The result is that, in general, the partition function can not be evaluated
exactly \cite{Landau}.\\[1.5mm]
%
\indent The Monte Carlo approach consists of generating a series of
possible states or configurations $X_{1},X_{2},...,X_{N}$ of a
system ($X_{i}=\{ x_{1}, x_{2} ... \}$ with $x_{i}$ being the
position of the particles in the system), so that the probability
$P_{X_{i}}$ of encountering the system in state $X_{i}$, is given by
an appropriate probability density function. Averages over phase
space may be constructed by considering a large number of identical
systems which are held at the same fixed conditions. These are
called {\bf ensembles}, (Fig. \ref{fig:ensemble}), and depending on
the parameters held fixed, one can have different types of
ensembles. In the case in which $T$ is maintained constant, the set
of systems obtained is said to belong to the canonical ensemble, in
which the systems are allowed to have distinct energies. On the
other hand, if the energy is fixed, the ensemble is called the
microcanonical ensemble. In both cases the number of particles is
also fixed, but if now we allow the number of particles to
fluctuate, the ensemble is named the grand canonical ensemble
\cite{Landau}.
%
\begin{figure}[h]
\begin{center}
\resizebox{50mm}{!}{\includegraphics{ensemble.ps}}
\caption{Graphical representation of a canonical ensemble: the
positions of the particles and the energy can change in each system,
but the number of particles and the temperature is fixed.}
\label{fig:ensemble}
\end{center}
\end{figure}\\[1.5mm]
%
\indent
In the canonical approach, $Z(H,T)$ is calculated in the following way:
\begin{equation} \label{eq:z}
Z(H,T)=\sum_{all \, states} e^{-H/k_{B}T},
\end{equation}
where $k_{B}$ is the Boltzmann's constant, $H$ denotes the
Hamiltonian and $T$ the temperature of the system. By all states we
mean taking into the sum all the available configurations for the
system. The probability distribution is called a canonical
distribution if it is given according to the equation:

\begin{equation} \label{eq:proba}
P_{X}= \frac{e^{-H(X)/k_{B}T}}{Z(H,T)}.
\end{equation}

The general goal is to determine equilibrium properties of the canonical ensemble such as energy and magnetization. If $m(X)$ is the value of some
physical property in a state $X$, and $H(X)$ the energy of this state, then the canonical ensemble average for the quantity $m$ is given by:

\begin{equation} \label{eq:aver}
\langle m \rangle=\frac{\sum_{all \, states} m(X)e^{-H(X)/k_{B}T}}{Z(H,T)}.
\end{equation}

As mentioned before, the problem is how to calculate $Z(H,T)$ in an efficient way.\\[1.5mm]
%
\indent If we have a finite state space $\mathcal{X}$, where
$X_{(t)}$ is the state of the system at time $t$, that can only take
$s$ discrete values $X_{(i)} \in  \mathcal{X} = \{
X_{1},X_{2},...,X_{s}\}$, the stochastic process is called a Markov
chain if the following condition is fulfilled:
%
\begin{equation*}
P(X_{(t)}|X_{(t-1)},...,X_{(1)})=T_{M}(X_{(t)}|X_{(t-1)}),
\end{equation*}
%
where $P(X_{(t)}|X_{(t-1)},...,X_{(1)})$ is the probability of the state $X_{(t)}$ to occur conditioned by the occurrence of the past
states $X_{(t-1)},...,X_{(1)}$. $T_{M}$ is known as the transition probability matrix. The chain is homogeneous if the transition
probability $T_{M}=T_{M}(X_{(t)}|X_{(t-1)})$ is constant for all $t$, with $\sum_{X_{(t)}} T_{M}(X_{t}|X_{(t-1)})=1$ for any $t$. That is,
the evolution of the chain in the state space $\mathcal{X}$ depends solely on the current state of the chain and a fixed transition (probability)
matrix \cite{Freitas}.\\[1.5mm]
%
\indent
For any starting point, the chain will converge to an invariant distribution $P(X)$, as long as $T_{M}$ is a stochastic transition matrix
with the following properties:

\begin{enumerate}
\item { \it Irreducibility}: for any state of the Markov chain, there is a positive probability of visiting all other states. That is, the
matrix $T_{M}$ can not be reduced to smaller matrices, which is also the same as stating that the transition graph is connected.
\item { \it Aperiodicity}: the chain should not get trapped in cycles \cite{Freitas}, i.e., the system should not be limited to a
subchain of states.
\end{enumerate}

Consider now a large collection of copies of the same system in
equilibrium. We allow each copy to evolve in time and, at any
instant, we will find each different copy in one possible
configuration, an all the copies will give a probability
distribution over the configuration space. For each point $X_i$ in
the configuration space, the probability $P$ of finding a copy in
$X$ at time $t$ satisfies the equation:

\begin{equation} \label{eq:mastereq}
\frac{d}{dt} P(X,t) = \sum_{i}[P(X_{i},t)T_{M}(X_{i} \rightarrow X)-P(X,t)T_{M}(X \rightarrow X_{i})].
\end{equation}

$T_{M}(X \rightarrow X_{i})$ and $T_{M}(X_{i} \rightarrow X)$ are the probabilities of making a transition from the configuration $X$ to $X_{i}$
and viceversa. Because the collection is in equilibrium, the probability distribution is time invariant, and in the last equation we must
have $d P(X,t)/dt=0$ for all $t$. At any instant, there is an equal number of transitions to and from the configuration $X$. In fact, there exists
an equation like \eqref{eq:mastereq} for each point in the configuration space, and the set of all such equations forms the master
equation \cite{Sun}.\\[1.5mm]
%
\indent A sufficient (but not necessary) condition for an
equilibrium (time independent) probability distribution needed to
simulate equilibrium systems is the so-called { \bf detailed balance
condition} for the master equation that relates the transition
between two configurations, $X_{n-1}$ and $X_{n}$ through:

\begin{equation}\label{eq:detbal}
P(X^{n})T_{M}(X^{(n-1)}|X^{(n)})=P(X^{(n-1)})T_{M}(X^{(n)}|X^{(n-1)}).
\end{equation}

This method can be used for any probability distribution of
configurations. If we choose the Boltzmann distribution, for which
the probability of finding a configuration $X$ with energy $H$ at
equilibrium is given by \eqref{eq:proba}, and substitute it into
\eqref{eq:detbal}, we get:

\begin{equation}
\frac{T_{M}(X^{(n-1)}|X^{(n)})}{T_{M}(X^{(n)}|X^{(n-1)})}=\frac{e^{-H(n-1)/k_{B}T}}{e^{-H(n)/k_{B}T}}= e^{ \Delta E /k_{B}T}.
\end{equation}

This is the detailed balance condition on the transition probabilities. It is very important to note that $Z(H,T)$ does not
appear in this expression; it only involves quantities that we know $(k_{B}T)$ or that can be easily calculated $(E)$. \\[1.5mm]
%
\indent Thus, we have a valid Monte Carlo algorithm if we generate a
new configuration $X_{(n)}$ from a previous one $X_{(n-1)}$ such
that the transition probability satisfies the detailed balance
condition, and the generation procedure is ergodic, i.e. every
configuration can be reached from every other configuration in a
finite number of iterations \cite{markov}.

\section{Measurements Using the Monte Carlo Method}

Systems generated using a valid Monte Carlo algorithm are often held at fixed values of intensive variables, such as temperature, pressure,
and so on. The corresponding conjugate extensive variables (energy, volume, etc.) will fluctuate in time; indeed these fluctuations will actually
be observed during the Monte Carlo simulations and will help us to measure quantities of interest such as:\\[1.5mm]
%
\indent
{\em Specif\mbox{}ic heat}
\begin{equation}
C_V= \frac{1}{V} \left( \frac{\partial E}{\partial T} \right)_{V}= \langle (E-\langle E \rangle)^2 \rangle = \langle E^2 \rangle -
\langle E \rangle^2 .
\end{equation}

{\em Susceptibility}
\begin{equation}
\chi = \frac{1}{V} \left( \frac{\partial M}{\partial T} \right)_V= \langle (M-\langle M \rangle)^2 \rangle = \langle M^2 \rangle -
\langle M \rangle^2 .
\end{equation}

These and other similar quantities are measured for each configuration and the averages and statistical errors calculated \cite{Landau}. \\[1.5mm]
%
\indent
Summarizing, the idea of Monte Carlo simulations is to create an independently and identically distributed set of $N$ samples from a target
density $P(X)$ distribution function defined on a high dimensional state space $\mathcal{X}$ (e.g., the set of possible configurations of a system).
These $N$ samples can be used to approximate $P(X)$ \cite{Freitas}.\\[1.5mm]
%
\indent
When $P(X)$ has a standard form, e.g., Gaussian, it is straightforward to sample from it using easily available routines. However, when this
is not the case, we need to introduce more sophisticated techniques such as Markov Chain Monte Carlo (MCMC) briefly presented above, which
is a strategy of generating samples using a Markov chain mechanism while exploring the state space $\mathcal{X}$. This mechanism is constructed
with the condition that the chain spends more time in the most important regions. In particular, it is constructed so that the samples mimic
samples drawn from the target density distribution $P(X)$ \cite{Freitas}.

%Since the number of dif\mbox{}ferent states is so huge, we are not only interested in probabilities of individual states but also in probabilities of macroscopic variables, such as the internal energy U. We f\mbox{}irst form the moments (where $\beta=1/k_{B}T$;)

%\begin{equation} \label{eq:uprom}
%\bar U(\beta)=\langle H(i) \rangle = \sum_{i}P_{(i)}H(i)=\frac{\sum_{i}H(i)e^{-\beta %H(i)}}{\sum_{i}e^{-\beta H(i)}},
%\langle H^{2} \rangle = \frac{\sum_{i}H^{2}e^{-\beta H(i)}}{\sum_{i}e^{-\beta H(i)}}
%\end{equation}

%and note the relation $-(\partial U(\beta)/ \partial \beta)_{V}= \langle H^{2} \rangle %-\langle H \rangle^{2}$. Since $-(\partial U/ \partial T)_{v}= C_{V}$ the specif\mbox{}ic heat %thus yields a f\mbox{}luctuation relation:


%\begin{equation} \label{eq:ces}
%k_{B}T^{2}C_{V} = \langle H^{2} \rangle - \langle H \rangle^{2}= \langle (\Delta U)^{2} %\rangle_{NVT}, \qquad \Delta U = H - \langle H \rangle.
%\end{equation}

%Now for a macroscopic system (number of particles $ N \rightarrow \infty $ ) away from a %critical point, $U \propto N$ and the energy and specif\mbox{}ic heat are extensive quantities. %However since both $\langle H^{2} \rangle$ and $\langle H \rangle^{2}$ are clearly %proportional to $N^{2}$, we see that the relative f\mbox{}luctuations of the energy is very small, %of order $1/N$. while in real experiments, where $N \rightarrow 10^{22}$, such f\mbox{}luctuations %may be too small to be detectable,chain in simulations these thermal f\mbox{}luctuations are readily %observable, and relations such as equation \eqref{eq:ces} are useful for the actual %estimation of the specif\mbox{}ic heat from energy f\mbox{}luctuations. Similar f\mbox{}luctuations relations %exist for many other quantities.

%\noindent
%o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o\\[1.5mm]

%\noindent
%Para mi:\\[1.5mm]

%It is intuitive to introduce Markov chains on f\mbox{}inite state spaces, where $x^{(i)}$ can only %take $s$ discrete values $x^{(i)} \in X = \{ x_{1},x_{2},...,x_{s}\}$. The stochastic %process $x^{(i)}$ is called a Markov chain if: \\[1.5mm]

%$p(x^{(i)}|x^{(i-1)},...,x^{(1)})=T(x^{(i)}|x^{(i-1)}).$\\[1.5mm]

%The chain is homogeneous if $T=T(x^{(i)}|x^{(i-1)})$ remains invariant for all $i$, with %$\sum_{x^{(i)}} T(x^{i}|x^{(i-1)})=1$ for any $i$. That is, the evolution of the chain in a %space $X$ depends solely on the current state of the chain and a f\mbox{}ixed transition matrix.\\[1.5mm]

%For any starting point, the chain will convergence to the invariant distribution $p(x)$, as %long as $T$ is a stochastic transition matrix that obeys the following properties:

%\begin{enumerate}
%\item Irreducibility: for any state of the Markov chain, there is a positive probability of %visiting all other states. That is, the matrix $T$ can not be reduced to separate smaller %matrices, which is also the same as stating that the transition graph is connected.
%\item Aperiodicity: the chain should not get trapped in cycles.
%\end{enumerate}

%A suf\mbox{}f\mbox{}icient, but not necessary, condition to ensure that a particular $p(x)$ is the %desired invariant distribution is the following reversibility (detailed balance) %condition:\\[1.5mm]

%$p(x^{i})T(x^{(i-1)}|x^{(i)})=p(x^{(i-1)})T(x^{(i)}|x^{(i-1)}).$\\[1.5mm]

%Summing both sides over $x^{(i-1)}$, give us\\[1.5mm]

%$p(x^{i})=\sum_{x^{(i-1)}}p(x^{(i-1)})T(x^{(i)}|x^{(i-1)}).$\\[1.5mm]

%MCMC samplers are irreducible and aperiodic Markov chains that have the target distribution %as the invariant distribution. One way to design these samplers is to ensure that detailed %balance is satisf\mbox{}ied. However, it is also important to design samplers that converge %quickly.\\[1.5mm]

%In continuous state spaces, the transition matrix T becomes an integral kernel K and p(x) %becomes the corresponding eigenfunction\\[1.5mm]

%$\int p(x^{(i)})K(x^{(i+1)}|x^{(i)})dx^{(i)}= p(x^{(i+1)}).$\\[1.5mm]

%The kernel $K$ is the conditional density of $x^{(i+1)}$ given the value $x^{i}$. It is a %mathematical representation of a Markov chain algorithm.\\[1.5mm]
%o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-o-\\[1.5mm]

\section{Ising and Potts Models}

The Ising model was proposed in 1925, in the doctoral thesis of Ernst Ising, a student of Wilhelm Lenz \cite{Ising}. Using a model proposed
by Lenz in 1920 \cite{Lenz}, Ising tried to explain certain empirically observed facts about ferromagnetic materials in his thesis.
The model was referred to in a paper by Heisenberg of 1928 in which he used the exchange mechanism to describe ferromagnetism \cite{Heisenberg}.
After the publication of a paper by Peierls (1936) \cite{Peierls}, in which he gave a non-rigorous proof that spontaneous magnetization must
exist, the Ising model became a well-established paradigm. In 1941, Kramers and Wannier calculated the Curie temperature using a two-dimensional
Ising model \cite{Kramers} and three years later Onsager gave a complete analytic solution of the model \cite{Onsager}.\\[1.5mm]
%
\indent
As a paradigm of statistical mechanics, the Ising model tries to imitate systems in which individual elements
(e.g., atoms, animals, protein folds, biological membrane, social behaviour, etc.) modify their behaviour so as to conform to the dynamics of
other elements in their neighbourhood \cite{Isingmodel}.\\[1.5mm]
%
\indent
In most specific terms, the Ising model in statistical mechanics considers a system with spins located at the sites of a D-dimensional lattice,
where each spin can take the value +1, corresponding to spin up, or the value -1, corresponding to spin down. The Hamiltonian of such a spin
lattice system is given by:

\begin{equation} \label{eq:isingB}
H_I= -J \sum_{\langle i,j \rangle} \sigma _{i} \sigma_{j} -B\sum_{i}\sigma_{i},
\end{equation}
where $J$ is the exchange constant, and $\sigma _{i}$ and $\sigma
_{j}$ are the spins of the $i^{th}$ and $j^{th}$ sites respectively.
The sites are usually a pair of nearest neighbours, though
calculations for more distant neighbours can also be carried out.
$B$ is an externally applied magnetic field with whom each spin
interacts.
%
\begin{figure}[h]
\begin{center}
\resizebox{90mm}{!}{\includegraphics{isiypot2.ps}} \caption{Lattice
representations of Ising and Potts models. The red site interacts
with his first neighbours (in yellow). Notice that in the Potts
model, being a generalization of the Ising model, more than two
possible directions for the spin are available.} \label{fig:ispott}
\end{center}
\end{figure}

When $J>0$, the model describes a ferromagnetic system where parallel spins are favoured and antiparallel spins are discouraged.\\[1.5mm]
%
\indent
In the case of $J<0$, an antiferromagnetic system is modeled.\\[1.5mm]
%
\indent
If $J$ is randomly chosen to be 1 or -1 for each pair of nearest neighbours and remain fixed during the course of observation, we obtain a model
of a spin glass \cite{Marinari}.\\[1.5mm]
%
\indent The energy associated with each state depends then on the
exchange energy of the particles and the interaction of the
particles with the external magnetic field. However, in the absence
of the external field, the energy of the system depends only on the
spin exchange energy:

\begin{equation} \label{eq:ising}
H_I= -J \sum_{\langle i,j \rangle} \sigma _{i} \sigma_{j}.
\end{equation}

The Potts model is a generalization of the Ising model, in which
spins can choose its value from a discrete set of states (see Fig.
\ref{fig:ispott}). In 1952, C. Domb proposed it as a doctoral thesis
for his student R. Potts \cite{Potts}. Without the presence of an
external field the Potts model is defined through the Hamiltonian:

\begin{equation} \label{eq:potts}
H_P= -J \sum_{\langle i,j \rangle} \delta_{\sigma_{i},\sigma_{j}} \sigma _{i} \sigma_{j},
\end{equation}
where $J$ denotes again the interaction exchange constant between
nearest neighbours and the values $ \sigma_{i} $ are characterized
by an integer  $\sigma_{i} = 1,2,...,q$. If two spins are parallel
they contribute with energy $J$, otherwise their energy contribution
is null.

\section{Some Monte Carlo Algorithms: Metropolis, Swendsen-Wang and Wolff}

The Metropolis \cite{MetroTeller}, Swendsen-Wang \cite{SwendsenWang} and Wolff \cite{Wolff1} algorithms satisfy the master equation and the
detailed balance condition for the Boltzmann distribution. Consequently, when the system reaches equilibrium, the probability distribution of
all possible configurations will be the Boltzmann distribution.\\[1.5mm]
%
\indent The steps of the Metropolis algorithm for an Ising model are
graphically represented in Fig. 1.7 and are the following:

\begin{enumerate}
\item Start with an arbitrary spin configuration $C_{0}$ of a lattice with $N$ sites.
\item Select a spin randomly and independently, and flip it.
\item Calculate the energy change $\Delta E$ which results if the spin is turned.
\item Generate a random number $r$ such that $0<r<1$.
\item If $\Delta E \leq 0$, accept the change; if $\Delta E > 0$, the configuration is accepted with a
probability $e^{-\Delta E / k_{B}T}$. This is resumed as: if $r <
e^{-\Delta E / k_{B}T}$ the spin is flipped. If not, the new
configuration is rejected, and the system returns to the initial
configuration $C_{0}$.
\item Choose randomly another spin to flip and go to (3).
\end{enumerate}


\begin{figure}[h]
\hfill
\begin{minipage}[t]{3.8cm}
\includegraphics[width=0.9\textwidth]{metro1.ps}
\end{minipage}
\begin{minipage}[t]{3.8cm}
\includegraphics[width=0.9\textwidth]{metro2.ps}
\end{minipage}
\hfill
\begin{minipage}[b][4.0cm][s]{5.0cm}
\caption{Metropolis algorithm: If the energy decreases with the spin
flip, the new configuration remains. If not, is accepted or rejected
with certain probability.}
\end{minipage}
\hfill
\label{fig:met}
\end{figure}

It is important to discard some configurations at the beginning of the chain of configurations to ensure that the system forgets $C_{0}$ and
that the configurations taken into account form a canonical ensemble. Then, after a considerable number of spins have been updated, the properties
of the system are determined and added to the statistical average which is stored. The random number $r$ must be chosen uniformly in the
interval $[0,1]$ and all the successive random numbers should be uncorrelated. Note that if a spin trial is rejected, the old state is counted
again for the averages. For a $q$ state Potts model, the new value for the chosen spin is selected randomly among the other $q-1$ spin
values \cite{Landau}.\\[1.5mm]
%
\indent In the Metropolis algorithm, spins are updated one at a time
and this single spin flip is the reason why this algorithm is
inefficient at critical points where the phenomenon of slowing down
occurs. The standard measure of Monte Carlo time is the Monte Carlo
step per site (MCS/site), which corresponds to $N$ trial flips,
regardless of whether the trial is successful or not ($N$ is the
total number of spins in the
system) \cite{Sun}.\\[1.5mm]
%
\indent
The Swendsen-Wang and Wolff algorithms are cluster algorithms, where groups of spins are identified by establishing bonds between pairs of
neighbouring spins. Once the clusters in the lattice are identified, a whole spin cluster is updated, and in this way these algorithms are more
efficient near critical points.\\[1.5mm]
%
\indent The Swendsen Wang algorithm for a $q$ state Potts model is
(Fig. \ref{fig:swd}):

\begin{enumerate}
\item Initialize the lattice of $N$ sites with an arbitrary spin configuration $C_{0}$.
\item Examine every pair of neighbouring spins in the system. If neighbouring spins are not parallel, nothing is done. If they are
parallel, a bond is introduced between them with probability $p=1-e^{-K}$, where $K=J/k_{B}T$. (If $p<1$, a random number $r$ is generated
such that $0<r<1$, and if $r<p$ a bond is introduced between sites $i$ and $j$).
\item Once all clusters in the lattice have been formed, an arbitrary cluster is chosen.
\item Another random number $R$ is generated such that $1 \leq R \leq q$.
\item All spins in the chosen cluster are assigned $\sigma_{i}=R$.
\item Another cluster is selected randomly and return to (4).
\item When all clusters have been considered, erase the bonds, go to (2) and repeat the steps until the desired number of configurations
has been obtained.
\end{enumerate}


\begin{figure}[h]
\begin{minipage}[t]{3.5cm}
\includegraphics[width=0.9\textwidth]{swd1.ps}
\end{minipage}
\hfill
\begin{minipage}[t]{3.5cm}
\includegraphics[width=0.9\textwidth]{swd2.ps}
\end{minipage}
\hfill
\begin{minipage}[t]{3.5cm}
\includegraphics[width=0.9\textwidth]{swd3.ps}
\end{minipage}
\hfill
\begin{minipage}[t]{3.5cm}
\includegraphics[width=0.9\textwidth]{swd4.ps}
\end{minipage}
\hfill \caption{Swendsen-Wang algorithm: Once the clusters are
formed (each one is represented by a diferent colour), their spin
values are randomly modified. Some clusters maintain the same value
(i.e., orange spin). After that, the cluster formation starts
again.} \label{fig:swd}
\end{figure}

One Monte Carlo cycle in the Swendsen-Wang algorithm is accomplished when all clusters have been updated (steps 2-6), and is equivalent to one
Monte Carlo step per site (MCS/site) in the Metropolis algorithm \cite{Sun}. \\[1.5mm]
%
\indent
The probability to set a bond between two sites depends on the temperature, which affects the resultant cluster distribution. At very
high temperature, the clusters will tend to be quite small, whereas at very low temperature virtually all sites with nearest neighbours in
the same state will belong to the same cluster and therefore there will be a tendency for the system to oscillate back and forth between quite
 structures. However, near a critical point, a quite rich array of clusters is produced and the net result is that each configuration differs
 substantially from its previous one. That is the main reason why the critical slowing down is reduced \cite{Landau}. \\[1.5mm]
%
\indent The Wolf\mbox{}f algorithm is very similar to the
Swendsen-Wang algorithm, the principal difference being that it
f\mbox{}lips the spins of one particular cluster with the maximum
probability of 1 in each Wolff MC cycle. The Wolff algorithm was
proposed to improve the Swendsen Wang algorithm in which significant
effort is required in dealing with small clusters as well as large
ones. However, the small clusters do not contribute to the critical
slowing down \cite{Landau} and can be disregarded. The Wolff
algorithm is given by the following procedure (a graphical
representation is provided in Fig. \ref{fig:wolff}):

\begin{enumerate}
\item Start with an arbitrary spin configuration $C_{0}$ of a lattice with $N$ sites.
\item Randomly choose a spin to be the seed of a cluster.
\item Examine all its neighbours and draw bonds with probability $p=1-e^{-K \delta_{i}\delta_{j}}$.
\item If bonds have been drawn to any nearest neighbour site $j$, draw bonds to all nearest neighbours $k$ of site $j$ with
probability $p=1-e^{-K \delta_{j}\delta_{k}}$.
\item Repeat step (4) until no more new bonds are created.
\item Flip all spins in the cluster to a different randomly chosen spin value.
\item Go back to (1).
\end{enumerate}

The measurement of Monte Carlo time is more complicated. The natural
unit of time is the number of cluster flips. However, in one cluster
flip the number of spins visited is not equivalent to the total
number of spins in the system and hence one Wolff cluster flip is
not equivalent to one MC step per spin (MCS/site) or one MC cycle in
the Metropolis and Swendsen-Wang algorithms. The generally accepted
method of converting to MCS/site is to normalize the number of
cluster flips by the mean fraction of sites $\langle c \rangle$
flipped at each step. The Monte Carlo time then becomes well defined
if $\langle c \rangle$ is well defined, and this happens only after
enough flips have occurred \cite{Landau}.

\begin{figure}[h]
\begin{minipage}[t]{3.5cm}
\includegraphics[width=0.9\textwidth]{wol1.ps}
\end{minipage}
\hfill
\begin{minipage}[t]{3.5cm}
\includegraphics[width=0.9\textwidth]{wol2.ps}
\end{minipage}
\hfill
\begin{minipage}[t]{3.5cm}
\includegraphics[width=0.9\textwidth]{wol3.ps}
\end{minipage}
\hfill
\begin{minipage}[t]{3.5cm}
\includegraphics[width=0.9\textwidth]{wol4.ps}
\end{minipage}
\hfill \caption{Wolff algorithm: A spin is chosen randomly, and the
cluster is formed from it by introducing bonds to its neighbours and
the neighbours of its neighbours with some given probability. The
spin value of the cluster is changed and then another spin is
selected to start a new cluster.} \label{fig:wolff}
\end{figure}

Although all these algorithms satisfy detailed balance, they do not give the same results for $M$ and $\chi$ in a simulation. This difference is due
to the very small probability for $M$ to change sign using the Metropolis algorithm for large systems, at low temperatures. This corresponds
to a physical situation, and one can calculate $\langle M \rangle$ and $\chi$ and obtain meaningful results. However in cluster algorithms,
the clusters become very large at low temperatures, and by flipping them, we effectively flip the whole system, yielding $\langle M \rangle = 0$;
the variance in $M$ is then simply $\langle M^{2}\rangle$, a constant at low temperatures, which in turn gives a
diverging $\chi _{M}$ as $T \rightarrow 0$. The solution is to use $|M|$ instead of $M$, and define $\chi _{|M|}$ just as we defined $\chi$ earlier.
In this way, all three algorithms give the same results for $\langle M \rangle$ and $\chi _{|M|}$ at all temperatures \cite{Sun}.\\[1.5mm]
%
\indent
Notice that cluster algorithms become inefficient at low temperatures, because in that situation, nearly all spins in the system are flipped when
we flip the largest cluster, which is not helpful in achieving statistically independent configurations. In comparison, the Metropolis
algorithm will be much more efficient \cite{Sun}.\\[1.5mm]
%
\indent
Once an appropiate algorithm has been selected, one of the goals of Monte Carlo simulations is the study of the behaviour of systems in
phase transitions.

\section{Phase Transitions and Critical Exponents}

One of the most common physical problems studied in simulations are phase transitions. A phase transition occurs when a thermodynamic system
passes from one phase to another one with the change of some external variable, such as temperature or pressure. Some examples are the transitions
between solid, liquid, and gaseous phases, the transition between the ferromagnetic and paramagnetic phases of magnetic materials, and the emergence
 superconductivity in certain metals when they are cooled below a critical temperature \cite{phtrwiki}.\\[1.5mm]
%
\indent
When a system goes from one phase to another, there will be in general a stage where the free energy is not analytic. Due to this, the
free energies on either side of the transition are two different functions, so one or more thermodynamic properties will behave very differently
after the transition. A system near or at the critical point of a  phase transition presents peculiar behaviours that are universal, like
divergence of some quantities and critical slowing down phenomena, which will be explained later. The most commonly examined property in this
context is the heat capacity that in the transition region may become infinite, jump abruptly to a different value, or exhibit a discontinuity in
its derivative \cite{phtr}. This non-analytic behaviour stems generally from the interactions of an extremely large number of particles in a system,
and does not show up with the same strength in systems that are too small \cite{phtrwiki}.\\[1.5mm]
%
\indent Phase transitions are generally classified into first or
second order transitions. A second order, or continuous phase
transition, can be defined as a point at which a system changes from
one state to another one without a discontinuity or jump in its
density, internal energy, magnetization, or similar properties. In
the case of a first order transition, the above mentioned properties
jump discontinuously as the temperature or pressure passes through
the transition point \cite{Critical}. The name of different kind of
phase transitions comes precisely from the number of derivatives of
the free energy that we have to count before we can see a
discontinuous behaviour. If the first derivative is discontinuous,
we have a first order transition, if not, it is a second order one
\cite{Landau}.

The first-order phase transitions involve a latent heat. During such transition, a system either absorbs or releases a fixed (typically large)
amount of energy. Because energy can not be instantaneously transferred between the system and its environment, first-order transitions are
associated with ``mixed-phase regimes'' in which some parts of the system have completed the transition and others have not. Continuous phase
transitions, in many cases, are associated with a change of symmetry of the system and are easier to study than first-order transitions due to the
absence of latent heat. They have shown many interesting properties. The phenomena associated with continuous phase transitions are called
critical phenomena, because of their occurrence near critical points and because it turns out that continuous phase transitions can be characterized
by parameters known as critical exponents \cite{phtrwiki}.\\[1.5mm]
%
\indent
In the case of many phase transitions a non-zero value of an order parameter appears, i.e., some property of the system which is non zero in
one phase (usually called the ordered phase) but identically zero in the other phase (disordered phase). Thus, the order parameter can not be
an analytic function at the transition point. The order parameter is defined differently in various kinds of physical systems \cite{Landau}. For
systems such as the ferromagnet, where there is a broken symmetry below critical temperature $T_c$, the order parameter is the magnetization.
For systems without broken symmetry, one chooses some quantity that is very sensitive to the difference between the two phases, and measures the
difference of this quantity from its value at the critical point and below it. For the liquid-vapor critical point, we may choose the order
parameter as the difference between the actual density of the fluid and the density at the critical point. For liquid crystals the degree of
orientational order is considered as the order parameter \cite{Critical}.\\[1.5mm]
%
\indent
Another quantity of interest near a phase transition is the correlation function. In general, there will be microscopic regions in which
the characteristics of the material are correlated. This is generally measured through the determination of a {\em two point correlation function},
which is the probability of finding that two sites separated by a distance $r$ have the same value of a certain given quantity $\rho$ \cite{Landau}:
\begin{equation}\label{eq:corr}
\Gamma_{\rho}(r)=\langle \rho(0)\rho(r) \rangle.
\end{equation}
\indent
In the case of magnetic systems, the correlation function can be measured in neutron scattering experiments, whereas near the liquid vapour
transition it can be measured by light scattering or small angle X-ray-scattering experiments \cite{Critical}.\\[1.5mm]
%
\indent If the correlation for the appropriate quantity decays to
zero as the distance goes to infinity, then the order parameter is
zero \cite{Landau}. Close to the critical point, the correlation
length $\xi$, which tells us how far correlations are still present,
becomes extremely large. This is directly related to the large
amount of long-wavelength fluctuations that occur in the system at
the criticality \cite{Critical}. The time taken for the system to
change configuration near the critical point also increase
significantly because of the divergence of the correlation length
$\xi$. This phenomenon is called critical slowing down. For example,
in the case of the Ising model, spins tend to align with their
neighbours due to the exchange interaction, and regions or clusters
of spins pointing in the same direction appear. These spins are said
to be correlated, and, generally, there are clusters of various
sizes. The span of the largest one is the correlation length $\xi$,
while the time it takes to break up the existing conformation of
spins and form another arrangement of clusters is called the
decorrelation time $\tau$. At the critical point, there is a low
probability for a spin in the middle of a spin cluster to change its
direction, therefore spin regions are altered only at the boundary.
This gives rise to a long decorrelation time which is related to the
correlation length by a power law:
\begin{equation} \label{eq:slow1}
\tau \propto \xi ^{z},
\end{equation}
where $z$ is the dynamical critical exponent \cite{Sun}. For
simulations of a finite lattice of linear dimension $L$, $\xi$ is
naturally bounded by $L$ and then the basic assumption is that:
\begin{equation}\label{eq:slow2}
\tau \propto L^{z}.
\end{equation}

These two equations describe the critical slowing down. In an infinite system, as the critical point is approached, the correlation length
diverges (its value is $\infty$), and from \eqref{eq:slow1}, we see that the decorrelation time also diverges. In finite systems $\xi$ does not
diverge as the critical point is approached, however, it reaches its peak with a sharp slope. Due to the power law
dependence of $\tau$ on $\xi$, $\tau$ will also display a peak with a sharp slope, exhibiting critical slowing down \cite{Sun}.\\[1.5mm]
%
\indent
Near the transition points, the critical slowing down phenomenon produces important effects that complicate the implementation of the Monte Carlo
method. This is the main reason why the scientists introduced alternative approaches besides canonical Metropolis algorithm, such as Wolff and
Swendsen-Wang algorithms. The computational effect of critical slowing down near a critical point can be understood in the following manner:
when we simulate finite systems at the critical point, the decorrelation time depends on the linear dimension $L$ through a power law
as $L$ approaches infinity. Take, for example, the 2D Ising model. The dynamical critical exponent $z$ is known to be approximately 2 using
the Metropolis algorithm. If the time it takes to obtain 100 statistically independent configurations is $t$ in a system with $L=32$, then
if $L$ is increased by a factor of 2 to 64, the computational time needed to obtain 100 statistically independent configurations will increase
to $4^{2}\,t$. A factor of 4 is introduced because the number of spins is increased by 4, and another factor of 4 is due to the fact
that $\tau \propto L^{2}$. In general, the amount of CPU time required to obtain a fixed number of statistically independent configurations for a
system with linear dimension $L$ is proportional to $L^{d+z}$, where $d$ is the spatial dimension of the model, and $z$ is the corresponding
dynamical critical exponent \cite{Sun}.\\[1.5mm]
%
\indent Data from experiments, as well as results for a number of
exactly solvable models, show that in the vicinity of the critical
point $T_c$, the thermodynamical properties can be described by a
set of simple power laws \cite{Landau}. For example, for the
determination of the way
 which the magnitude of the order parameter
approaches zero as the critical point is reached, we may write
(according to the classical theories of phase transitions such as
the van der Waals or mean field theories):

\begin{equation}\label{eq:beta}
M=M_{0}\,\epsilon^{\beta},
\end{equation}
where $M$ is the order parameter (i.e., the magnetization for a ferromagnet), $M_{0}$ is a constant that will vary from one system to
another, $\epsilon = |1-T/T_{c}|$, and the exponent $\beta$ is called critical exponent \cite{Critical}.\\[1.5mm]
%
\indent The temperature variation of the order parameter is very
important but not the only quantity of interest. Another key
quantity is the specific heat, defined as the derivative of the
internal energy with respect to the temperature. The specific heat
is found to become infinite at the critical point in some systems
but also one can have cases in which the specific heat is finite
with only a sharp cusplike maximum at the critical point
\cite{Critical}. In either case, one may define an exponent $\alpha$
that characterizes the anomalous behaviour of the specific heat at
the critical point:
\begin{equation}\label{eq:alpha}
C_{V}=C_{0}\,\epsilon^{-\alpha}.
\end{equation}

Susceptibility $\chi$ is another quantity of interest. It is defined
as the derivative of the order parameter with respect to the applied
field to which it is coupled, under constant temperature condition.
For a magnetic system, this quantity is precisely the magnetic
susceptibility. This quantity becomes extremely large near the
critical point, and we may write the zero field magnetic
susceptibility as \cite{Critical}:

\begin{equation}\label{eq:gamma}
\chi= \chi _{0}\,{\epsilon}^{-\gamma}.
\end{equation}

Finally, the correlation length $\xi$ varies as:

\begin{equation}\label{eq:xi}
\xi = \xi_{0}\,{\epsilon}^{-\nu},
\end{equation}
where, again, $\nu$ is termed as critical exponent.\\[1.5mm]
%
\indent
Note that the last equations represent asymptotic expressions which are only valid if $\epsilon \rightarrow 0$ and more complete forms would
include additional corrections to scaling terms which describe the deviations from the asymptotic behaviour. The exact values of these critical
exponents are known exactly only for a small number of models, most notably for the 2D Ising square lattice \cite{Onsager}, whose exact solution
shows that $\alpha =0$, $\beta=1/8$, and $\gamma=7/4$. Here, $\alpha = 0$ corresponds to a logarithmic divergence of the specific
heat \cite{Landau}.\\[1.5mm]
%
\indent
The power law behaviour near critical points is very general and many systems share the same critical exponents. In particular, the Ising
universality class refers to the class of critical phenomena that share the same critical exponents as the Ising model \cite{Sun}.\\[1.5mm]
%
\indent Although the critical exponents, $\alpha$, $\beta$, and
$\gamma$ defined above may be independent in principle, they were
found empirically, in the 1960's, to be connected by the
relationship:
\begin{equation}\label{eq:rushbrooke}
\alpha = 2 - \gamma -2\beta.
\end{equation}

This equality is known as the Rushbrooke relation, and the following three relations are also known \cite{Landau}, where $\eta$
and $\delta$ are two additional critical exponents:

\begin{center}
\begin{tabular}[c]{lrcl}
Josephson: & $\nu D$& $=$ & $2-\alpha$,\\
Widom: & $\gamma$ & $=$ &$ \beta (\delta - 1)$ ,\\
Fisher: & $\gamma$ & $=$ & $\nu (2- \eta)$ .\\
\end{tabular}
\end{center}

In Table 1.1 we provide the theoretical values of the critical
exponents for $q \leq 4$ 2D Potts model, which of course fulfills
the latter relations.

\begin{table}[h]
\begin{center}
\begin{tabular}{| l || c | c | c | c | c | c |}
\hline
 & $\alpha$& $\beta$ & $\gamma$& $\nu$ & $\delta$ & $\eta$\\
\hline\hline
q=0& $- \infty $ & $1/6$ & $\infty$& $\infty$ & $\infty$ & $0$ \\
\hline
q=1& $-2/3$& $5/36$ & $2 7/18$& $4/3$ &$18 \, \, 1/5$ & $5/24$\\
\hline
q=2& $0$& $1/8$ & $7/4$& $1$ & $15$ & $1/4$\\
\hline
q=3& $1/3$& $1/9$ & $13/9$& $5/6$ & $14$ & $4/15$\\
\hline
q=4& $2/3$& $1/12$ & $7/6$& $2/3$ & $15$ & $1/2$\\
\hline
\end{tabular}
\caption{Some theoretical critical exponents for the 2D Potts model \cite{Wu}.}
\end{center}
\end{table}


The quantities discussed above are all equilibrium or static
quantities; they can be measured in a time-independent experiment in
thermal equilibrium conditions, and any involved correlation
function refers to the correlation of fluctuations at a single
instant of time. The majority of theoretical studies and experiments
on critical phenomena are concerned with these static measurements.
Thus, the usual division of systems into different universality
classes is based on these static phenomena. There are other
properties of systems, known as dynamical properties, which require
a more detailed theoretical analysis. Moreover, they require a
further subdivision of the universality classes. Two systems that
belong to the same universality class for their static properties
could show quite different behaviours in their dynamical properties.
Some standard examples of dynamical properties are various
relaxation rates of systems slightly disturbed from equilibrium,
correlations involving fluctuations at two different time instants,
and transport coefficients, e.g., thermal and electrical
conductivities. Among the experiments used for studying dynamical
properties we quote measurements of sound-wave attenuation and
dispersion, widths of nuclear and electron magnetic resonance lines,
and inelastic scattering experiments. Typically, one finds that the
relaxation rate of the order parameter becomes anomalously slow at a
critical point. However, some other relaxation rates are found to
speed up and transport coefficients become large in a number of
cases. In some cases, the results of a dynamical experiment may be
interpreted as an indirect measurement of a static property of the
system. As a matter of fact, some of the most precise measurements
of static critical properties have been obtained by dynamical means.
Examples are the measurements of the superfluid properties of liquid
helium, the low-frequency sound velocity of a fluid, and the
frequency of nuclear magnetic resonance in a magnetic system
\cite{Critical}.


\section{The Histogram Method}

The canonical Metropolis algorithm yields mean values of various thermodynamical quantities, (energy, magnetization, etc) at particular values of
the temperature $T$. Near a phase transition, many thermodynamical quantities change rapidly, and we need to determine these quantities at closely
spaced values of $T$. If we use standard Monte Carlo methods, we will have to do many simulations to cover the desired $T$ range \cite{Christian}.
The use of histograms to overcome this problem became popular after the publication of a paper by Ferrenberg and Swendsen in 1988 \cite{FerreSwend1}.
However, the histogram technique is one of the oldest techniques proposed \cite{histold, histold2}. Also often referred to as
Ferrenberg-Swendsen reweighting technique, is used in almost all Monte Carlo calculations of statistical physics, especially when dealing
with phase transition phenomena \cite{Venu}. The idea is to use the knowledge of the equilibrium probability distribution at one value
of $T$ (and other external parameters) to estimate the desired thermodynamical averages at neighbouring values.\\[1.5mm]
%
\indent A Monte Carlo simulation performed at $T=T_0$ generates
configurations of the system with a frequency proportional to the
Boltzmann weight, $e^{-\beta_{0}H}$, where $\beta_{0}=1/k_{B}T_{0}$,
and $H$ is the Hamiltonian of the system being studied. In the case
of a magnetic system, the probability of simultaneously observing
the system with energy $E$ and magnetization $M$ is given by:

\begin{equation}\label{eq:prohis}
P_{\beta_{0}}(E,M)= \frac{1}{Z(\beta_{0})} W(E,M)e^{-\beta_{0}E},
\end{equation}
where $W(E,M)$ is the number of configurations (density of states)
with energy $E$ and magnetization $M$, and $Z(\beta_{0})$ is the
partition function of the system. Because the simulation generates
configurations according to the equilibrium probability
distribution, a histogram $H(E,M)$ can be built during the
simulation to provide an estimate for the equilibrium probability
distribution that becomes exact in the limit of infinite-length run.
For a finite length-simulation, the histogram will present
statistical errors, but $H(E,M)/N$, where $N$ is the number of
measurements, still provides an estimate of $P_{\beta_{0}}(E,M)$
over the $E$ and $M$ values generated during the simulation
\cite{Felandau}. Keeping this in mind, we modify \eqref{eq:prohis}
as follows:

\begin{equation}\label{eq:prohis2}
H(E,M)= \frac{N}{Z(\beta_{0})} \tilde W(E,M)e^{-\beta_{0}E},
\end{equation}
where $\tilde W(E,M)$ is an estimate of the true density of states, or number of configurations, $W(E,M)$.\\[1.5mm]
%
\indent
The probability distribution for any value of $\beta$ has the same form as \eqref{eq:prohis}:

\begin{equation}\label{eq:progral}
P_{\beta}(E,M) = \frac{1}{Z(\beta)}W(E,M)e^{-\beta E}.
\end{equation}

Comparing \eqref{eq:prohis2} and \eqref{eq:progral}, we can note that it is possible to determine $\tilde W(E,M)$ from \eqref{eq:prohis2}:

\begin{equation}\label{eq:invert}
\tilde W(E,M) = \frac{Z(\beta_{0})}{N}H(E,M)e^{\beta_{0} E},
\end{equation}
and replace $W(E,M)$ in \eqref{eq:progral} with it. After
normalizing the distribution, we find that the relationship between
the histogram measured at $\beta=\beta_{0}$ and the (estimated)
probability distribution for an arbitrary $\beta$ is:

\begin{equation}\label{eq:relation}
P_{\beta}(E,M) = \frac{H(E,M) e^{-(\beta - \beta_{0})E}} {\sum_{E,M} H(E,M) e^{-(\beta - \beta_{0})E}}.
\end{equation}

From $P_{\beta}(E,M)$, the average value of any function $f(E,M)$ can be calculated as a continuous function of $\beta$:

\begin{equation}\label{eq:mean}
\langle f(E,M) \rangle _{\beta} = \sum_{E,M}f(E,M)P_{\beta}(E,M).
\end{equation}

The histogram method is useful only when the configurations relevant to the range of temperatures of interest occur with sufficient probability
during the simulation at temperature $T_0$. For example, if we simulate an Ising model at low temperatures at which only ordered configurations
occur (most spins aligned in the same direction), we can not use the histogram method to obtain meaningful thermodynamical averages at
 temperatures for which most configurations are disordered, and viceversa \cite{Christian}.\\[1.5mm]
%
\indent In the single histogram technique, the estimated $P(E,
\beta)$ is accurate only for $\beta$ close to the reference value
$\beta_{0}$. By generating many histograms that overlap each other
we can widen the range of $\beta$. This is called the multiple
histogram technique \cite{FerreSwend}. It is also clear that we can
increase the range of $\beta$ by directly estimating the density of
states $W(E,M)$. Multicanonical sampling \cite{BergN} is an early
technique proposed to do this. It is a very general and useful
technique being often the method of first choice for a variety of
problems that include critical slowing down near second order phase
transition points, nucleation in first order phase transitions, and
trapping in the metastable minima in systems with rugged energy
landscapes.

\section{Identifying the Nature of Transitions and Finite Size Scaling}

The behaviour near phase transitions has been one of the main objectives of studies focusing on the properties of physical systems but a
correlation length $\xi$ greater than the accessible size $L$ of the system may lead to many difficulties \cite{LeeKoster1}. For systems close to
a second order phase transition, finite-size scaling is routinely used to extract thermodynamic information from similar systems of fairly small
size. An equivalent theory for first order phase transitions is clearly also of interest. A useful theory of finite-size scaling should allow us to
extract the couplings at which the transition occurs, as well as other dimensional quantities like latent heat (or spontaneous magnetization)
and specific heat (or magnetic susceptibility) \cite{Gupta}.\\[1.5mm]
%
\indent
First order transitions are characterized by a discontinuity in the order parameter and thermodynamic quantities, with an associated
delta-peak behaviour in the susceptibility. As a matter of fact, the jump in the energy density is equivalent to the latent heat. However, at
finite size, thermodynamic quantities become continuous and rounded. Instead of delta function behaviour in susceptibility there is only a hump.
In simulations, this behaviour is visible only if the simulation time $\tau_s$ is larger than the decorrelation time $\tau$ at the transition
point. $\tau_s$ is typically very large since $\tau \propto e^{-\sigma2L^{D-1}}$, where $\sigma$ is the surface tension of the interface between
the low temperature and high temperature phases \cite{JCNiel}. It is the dimension $D$ that now plays the key role rather than the critical
exponents as in the case of second order phase transitions \cite{Landau}.\\[1.5mm]
%
\indent
At the transition temperature of a first-order phase transition, a mixed state can exist where two different bulk phases are separated by an
interface. The free energy densities of the two bulk phases are equal and the free energy of the mixed state is higher than any of the coexisting
pure phases by an amount $F_s = \sigma A$, where $A$ is the area of the interface and $\sigma$ is the interface tension \cite{Kanaya}.
In first order phase transitions, the correlation length remains finite in both the ordered and disordered phases, i.e., the correlation length
does not diverge. Thus, a different approach to finite size scaling must be used \cite{Landau}.\\[1.5mm]
%
\indent
From fairly general arguments about the nature of discontinuities at a first-order phase transition, Fisher and Berker \cite{FishBerk} obtained
the infinite volume limit approached by measurements performed at finite volumes.  This conventional scenario is based on a smooth behaviour of
the renormalization group flow and the existence of a discontinuity fixed point whose attraction domain contains the transition surface and has
relevant exponents of the form $y = D$ \cite{FishBerk}. The singularities associated with first order transitions are generated by infinite iterations
of renormalization group transformations in the thermodynamic limit. Correction terms were later calculated in a particular phenomenological
model called the double-Gaussian model, in which the peaks in the probability distribution for the coexisting phases were approximated by
Gaussians \cite{BinderLa, Challa}. This model correctly predicts the first term in a series of corrections in inverse powers of the volume $V$,
around the leading term obtained by Fisher and Berker \cite{FishBerk}. \\[1.5mm]
%
\indent
More recent developments are due to Borgs, Koteck\'y and Miracle-Sol\'e \cite{BorgsK, BorgsKM}. The basic idea is to decompose the partition
function into a sum of the contributions, each due to one of the coexisting phases, and to neglect contributions due to phase mixtures. Each of
these contributions to the total partition function then yield quantities related to free energies in the pure phases. The analysis proceeds by
power series expansions of these partial partition functions around the phase transition point, leading to moments expressed in inverse powers of
the volume \cite{Gupta}. According to this theory, for periodic boundary conditions, the specific heats and Binder cumulants at the transition
temperature can be represented by polynomials in $1/L^{D}$. If the $L >> \xi$, the contribution of the higher order terms are
negligible \cite{Billoire1,Burcu}. The difficulty arises when $\xi \geq L$. In this case, higher order corrections are necessary and deciding the
order of the transition becomes difficult. Even when large lattices are used, higher order terms may create difficulties during the fitting procedure
to the simulation data. Such difficulties may be reduced by choosing the quantities for which the correction terms play less important role.
A good example for such quantity is the average energy measured at the infinite lattice transition point, which has exponentially small
correction term enabling one to determine the infinite lattice critical point with great accuracy \cite{BorgsKM, Billoire1, BilloireLM}.\\[1.5mm]
%
\indent
Finite size scaling ideas for first or second order transitions help to extract critical exponents and other information, but this requires prior
knowledge of at least the nature of the transition. When the system undergoes a weak first order transition with $\xi >> L$, it becomes very
difficult to identify its nature even with large-scale computations. This problem is even worse when one encounters a system for which nothing
is known \cite{LeeKoster1, LeeKoster2}.\\[1.5mm]
%
\indent
Lee and Kosterlitz \cite{LeeKoster2} proposed a method which exploits the finite size scaling properties of the free energy $\Delta F(L)$.
These properties are unambiguous even when $\xi >> L$ and, more importantly, can be implemented with reasonable computational effort. This method
depends on two key ideas: the identification of $\Delta F(L)$, which has a characteristic behaviour as a function of $L$ at a first or second order
transition or in a single phase region, and the usage of histograms enabling this to be computed accurately. They have shown that the positions of
the peak free energies in a histogram should scale as $1/L$ if the system is well into the first order region. The ratio of $P(E)$ at its peaks
and minimum can be used to estimate an interface free energy $\Delta F(L)$, signaling a first order transition if it increases with system
size $L$. \\[1.5mm]
%
\indent This method uses the Helmholtz free energy $F$ of a system.
At low $T$, the low energy configurations dominate the contributions
to the partition function $Z$, even though there are relatively few
such configurations. At high $T$, the number of disordered
configurations with high $E$ is large, and hence high energy
configurations have a big contribution to $Z$. These considerations
suggest that it is useful to define a restricted free energy
$F_{r}(E)$ that includes only the main configurations at a
particular energy $E$:

\begin{equation}\label{Free}
F_{r}(E) = - kT \big[ \ln g(E) \big] e^{ -E/kT}.
\end{equation}

For systems with a first-order phase transition, a plot of
$F_{r}(E)$ versus $E$ will show two local minima corresponding to
configurations that are characteristic of the high and low
temperature phases. At low $T$, the minimum at the lower energy will
be the absolute minimum, whereas at high T the higher energy minimum
will be the absolute minimum of $F_{r}E$. At the transition
temperature, the two minima will have the same value of $F_{r}(E)$.
For systems with no transition in the thermodynamical limit, there
will only be one minimum for all $T$. How will $F_{r}(E)$ behave for
the relatively small lattices that we can simulate? In systems with
first-order transitions, the difference between low and high
temperature phases will become more pronounced as the system size is
increased. If the transition is continuous, there are domains at all
sizes, and we expect that the behaviour of $F_{r}(E)$ will not
change significantly while increasing the size. If there is no
transition, there might be a fake double minima for small systems
that disappear for larger systems \cite{Christian}. Lee and
Kosterlitz proposed the following method to classify phase
transitions:

\begin{enumerate}
\item Perform a simulation at a temperature close to the suspected transition temperature and calculate $H(E)$. Usually, the temperature at
which the peak in the specific heat occurs is chosen as the
simulation temperature.
\item Make use of the histogram method to calculate $F_{r}(E) \propto - \ln H_{0}(E) + (\beta - \beta_{0})E$ at neighbouring values of $T$.
If there are two minima in $F_{r}(E)$, vary $\beta$ until the values of $F_{r}(E)$ at the two minima are equal. The corresponding temperature is an
estimate of the possible transition temperature $T_c$.
\item The difference between the maxima and the minimum between the two peaks is used to estimate the free energy
barrier $\Delta F_{r}(E)$ at $T_{c}$.
\item Repeat steps (1-3) for larger systems. If $\Delta F_{r}(E)$ increases with size, the transition is first order. If $\Delta F_{r}(E)$ remains
the same, the transition is continuous. If $\Delta F_{r}(E)$ decreases and goes to zero with size, there is no thermodynamic transition.
\end{enumerate}

The above procedure is applicable when the phase transition occurs by varying the temperature. Transitions also can occur by varying the pressure
or the magnetic field. These field-driven transitions can be tested by a similar method. For example, consider the Ising model in a magnetic
field at temperatures below $T_c$. As we vary the magnetic field from positive to negative values, there is a transition from a phase with
magnetization $M >0$ to a phase with $M < 0$. Is this a first-order or continuous transition? To answer this question, we can use
the Lee-Kosterlitz method with a histogram $H(E,M)$ generated at zero magnetic field, and calculate $F_{r}(M)$ instead of $F_{r}(E)$.
The quantity $F_{r}(M)$ is proportional to $- \ln \sum_{E} H(E,M) e^{-(\beta - \beta_{0})E}$. Because the states with positive and negative
magnetization are equally likely to occur for zero magnetic field, we should see a double minima structure for $F_{r}(M)$ with equal minima.
As we increase the size of the system, $\Delta F_{r}$ should increase for a first order transition and remain the same for a continuous
transition \cite{Christian}.\\[1.5mm]
%
\indent Another way to determine the nature of a first order phase
transition is to use the Binder cumulant of energy defined by
\cite{Binder}:
\begin{equation}\label{eq:cumuo}
U_{L} = 1 - \frac{\langle E^{4} \rangle}{3 \langle E^{2} \rangle ^{2}} .
\end{equation}

If various cumulants (each one corresponding to different lattice
sizes) are plot in the same graph, a behaviour characteristic of a
first order transition appears as will be discussed in the next
section.

It can be shown that the minimum value of $U_{L}$ is

\begin{equation}\label{eq:cumumin}
U_{L,min} = \frac{2}{3} - \frac{1}{3} \Bigl( \frac{E_{+}^{2} - E_{-}^{2}}{2E_{+}E_{-}} \Bigl)^{2} + O(L^{-d}),
\end{equation}
where $E_{+}$ and $E_{-}$ are the energies of the two phases in a first order transition. These results are derived by considering the distribution
of energy values to be a sum of Gaussians about each phase at the transition point, which become sharper and sharper
as $L \rightarrow \infty$ \cite{Christian}.\\[1.5mm]
%
\indent On the other hand, equations \eqref{eq:beta} to
\eqref{eq:xi} for second order transitions are valid only for
infinite systems and, as a matter of fact, we can simulate only
finite systems. Quantities that diverge in the infinite case now
present peaks in the finite system. Furthermore, the peaks occur at
a value $T_{c}(L)$, for a given linear dimension $L$, slightly
different from the infinite-lattice critical temperature $T_c$.
However, at a second order phase change, the critical behaviour of a
system in the thermodynamical limit can be extracted from the
properties of finite systems by examining the size dependence of the
singular part of the free energy density. This finite size scaling
approach was first developed by Fisher \cite{Fisher}. According to
his theory, the free energy of a system of linear dimension $L$ is
described by the scaling ansatz:

\begin{equation}\label{eq:free}
F(L,T,h)=L^{-(2-\alpha)/\nu} F^{0}(tL^{1/\nu}, \quad hL^{(\gamma+\beta)/\nu}),
\end{equation}
where $t= (T-T_{c})/T_{c}$, $h$ is the magnetic field and $F^{0}$ is
a scaling function. The critical exponents $\alpha$, $\beta$,
$\gamma$, and $\nu$ all correspond to the values for the infinite
system. Appropriate differentiation of the free energy yields the
various thermodynamic properties with their corresponding scaling
forms:

\begin{equation}
\begin{array}{l}
m=L^{-\beta/\nu}\,m^{0}\,x_{t},\\
C=L^{\alpha/\nu}\,C^{0}\,x_{t},\\
\chi=L^{\gamma/\nu}\,\chi^{0}\,x_{t},\\
\end{array}
\end{equation}
where $x_{t}=tL^{1/\nu}$ is the temperature scaling variable \cite{Felandau}.\\[1.5mm]
%
\indent To determine the transition temperature accurately one
f\mbox{}ind the location of the peak in a thermodynamic derivative,
for example, specific heat. For a finite lattice the peak occurs at
the temperature where the scaling function $Z^{0}(x_{t})$ is
maximum, i.e., when

\begin{equation*}
\frac{dZ^{0}(x_{t})}{dx_{t}} \Biggl| _{x_{t}=x^{*}_{t}} = 0.
\end{equation*}

This temperature is the finite lattice (or effective) transition
temperature $T_{c}(L)$, defined through the condition $x_{t}=
x^{*}_{t}$ to vary with the lattice size, asymptotically, as:

\begin{equation*}
T_{c}(L)= T_{c}+ T_{c}x^{*}_{t}L^{-1/\nu}.
\end{equation*}

These results for the scaling of thermodynamic quantities and $T_{c}(L)$ are valid only for sufficiently large $L$ and temperatures
close to $T_{c}$. Corrections to finite size scaling must be taken into account for smaller systems. These are introduced as power law
corrections with an exponent $-w$, such that, for example, the magnetization at $T_{c}$ would scale with system size
like $L^{-\beta/\nu} (1+cL^{-w})$. As we move away from $T_{c}$, corrections to scaling due to irrelevant scaling fields, or nonlinearities in
the scaling variables must be introduced. Corrections due to irrelevant fields are expressed in terms of an exponent $\theta$ leading to
additional terms like $a_{1}t^{\theta} + a_{2}t^{2\theta}+..., $ while nonlinearities in the scaling variables give rise to corrections terms
of the form $b_{1}t^{1} + b_{2}t^{2}+..., $ \cite{Felandau}.\\[1.5mm]
%
\indent If we take one correction term into account, the estimate
for $T_{c}(L)$ is then modified in terms of the coupling
$K=J/k_{B}T$ as follows:

\begin{equation*}
K_{c}(L)= K_{c}+ \lambda L^{-1/\nu}(1+bL^{-w}).
\end{equation*}

Before this equation can be used to determine $K_{c}$, it is necessary to have an accurate estimate for $\nu$ and accurate values
for $K_{c}(L)$.\\[1.5mm]
%
\indent It has traditionally been difficult to determine $\nu$ from
Monte Carlo simulation data because of a lack of quantities which
provide a direct measurement. This situation was greatly improved by
Binder's introduction of the fourth order magnetization cumulant $U$
\cite{Binder} defined by:

\begin{equation} \label{eq:binderm}
U = 1 - \frac{\langle m^{4} \rangle}{3 \langle m^{2} \rangle^{2}},
\end{equation}
where $m$ is the magnetization per spin. Binder showed that the
slope of the cumulant at $K_{c}$, or anywhere in the finite size
scaling region, varies with system size like $L^{1/\nu}$. In
particular, the maximum value of the slope scales as $L^{1/\nu}$. If
we take into account a correction to scaling term, the size
dependence of the peak becomes:

\begin{equation*}
\frac{dU}{dK} |_{max} = aL^{1/\nu}(1+bL^{-w}).
\end{equation*}
\indent
The location of the maximum slope of $U$ also serves as an estimate for an effective transition coupling which can be used to
determine $K_{c}$. In the same paper, Binder introduced the cumulant crossing method which extracts a transition temperature by examining the
behaviour of the magnetization cumulant for different lattice sizes.\\[1.5mm]
%
\indent
Additional estimates for $\nu$ can also be obtained by considering the logarithmic derivative of any power of the magnetization, which has the
same scaling properties as the cumulant slope. The location of the maximum slope also provides an additional $K_{c}(L)$:

\begin{equation}\label{eq:deri}
\begin{array}{rcl}
\frac{\partial}{\partial K}\ln \langle m^{n}\rangle & = & \frac{1}{\langle m^{n} \rangle}\frac{\partial}{\partial K}\langle m^{n}\rangle \\
&=& \frac{\langle m^{n} E \rangle}{\langle m^{n}\rangle} - \langle E\rangle . \\
\end{array}
\end{equation}

To this end, the methods of finite size scaling are very helpful to
determine the behaviour of infinite systems from data obtained on
finite systems.

\section{Monte Carlo Simulations on the Betts Lattice}

Research of properties of lattices distinct from the commonly studied ones (square, triangular lattice) is a key step in the development and
prediction of the behaviour of possible new materials. A different lattice proposed by Donald Betts is constructed removing 1\textbackslash7 of
the sites in a two dimensional triangular lattice \cite{Betts}, accomplishing that each vertex has a coordination number of five and yielding
another translationally invariant lattice (see Fig.\ref{fig:maple}). This structure is known as Betts or Maple Leaf lattice, and lies between
the kagom\'e and triangular ones, which have coordination numbers of four and six, respectively. It has a hexagonal unit cell of six sites and
fifteen bonds, it is invariant under rotations through multiples of $60\,^{\circ}$, and, contrary to the kagom\'e and honeycomb lattices, it has no
inversion symmetry \cite{Richter}. To study the critical behaviour of this lattice, we performed Monte Carlo simulations using the Potts model
for $q=3$, $q=4$ and $q=5$.\\
\begin{figure}[h]
\begin{center}
\resizebox{12.0cm}{!}{\includegraphics{red.eps}}
\caption{Maple Leaf lattice}
\label{fig:maple}
\end{center}
\end{figure}

For the q-Potts model, the magnetization is defined as follows:
\begin{equation}\label{eq:mpotts}
m=\frac{N_{max}-1/q}{1-1/q}\,,
\end{equation}
where $N_{max}$ is the maximum number of equally oriented spins for certain configuration. We denote the lineal size of the system
studied as $L$, and this is related to the number of sites as $nsit=L\times L \times 6$. Earlier work has been already done on this lattice
for $q=3$, using the Metropolis algorithm, by Wang and Southern \cite{Wang}. We applied Wolff algorithm instead, due to its proved better
performance, and obtained similar results for ferromagnetic and antiferromagnetic cases. As predicted, calculations shown a second order
transition for the ferromagnetic case and a first order transition for the antiferromagnetic case. For $q=4$ and $q=5$ there is no published
work. We focus on the ferromagnetic regime in which the transition is found to be of second order for $q=4$ and of first order for $q=5$. In the
latter case, the transition is very weak and more calculations are needed to obtain better results.\\

\subsection{$q=3$, $J<0$:  Antiferromagnetic Case}

We selected four lattice sizes $L=12$, $18$, $24$ and $36$ to perform Monte Carlo simulations. The number of Monte Carlo steps used to
equilibrate the system before making the average was of the order of $2 \times 10^{5}$, and the number of steps used for averaging
was $6 \times 10^{5}$. Binder cumulants of the order parameter $E$ as a function of temperature for all lattice sizes demonstrate that the
system undergoes a first order transition, as each curve shown a deep minima whose value moves to lower temperature regions (Fig. \ref{fig:cumu}).
The critical temperature is obtained from the deep minimums showed by all curves, and its near $T_c=0.444$.\\[1.5mm]
%
\indent In Fig. \ref{fig:ce1q3}, specif\mbox{}ic heats for each
lattice size are plotted. There, the lattice size effect on the
results can bee clearly seen: the peaks are sharper and moves toward
smaller temperatures at larger lattice sizes. The transition
temperature can be estimated as the temperature where the peaks have
their maximum values, and obviously, the best approximation is
obtained for the largest lattice size.

\begin{figure}[h]
\begin{center}
\resizebox{10.0cm}{!}{\includegraphics{cumua.eps}} \caption{Energy
cumulants suggesting a first order phase transition for $q=3$,
$J<0$, $T_c=0.444$ and four lattice sizes.} \label{fig:cumu}
\end{center}
\end{figure}

\begin{figure}[h]
\begin{center}
\resizebox{10.0cm}{!}{\includegraphics{ce1q3a.eps}}
\caption{Specif\mbox{}ic heats for $q=3$, $J<0$ and the same four lattice sizes.}
\label{fig:ce1q3}
\end{center}
\end{figure}

\clearpage

Realizing that the phase transition appears to be of first order,
the next step is to calculate the energy distribution histograms
$P(E)$ for various lattice sizes near the estimated critical
temperature. We used $1 \times 10^{6}$ steps to equilibrate the
system and $4 \times 10^{6}$ steps for averaging. The histograms
always present two well-defined peaks, and while increasing $L$, the
minimum between the peaks becomes deeper. Moreover, the histograms
are sharper when more sites are taken into account (see Fig.
\ref{fig:hq3}). As explained in section 1.8, this is typical for
first order phase transition, confirming the nature of the
transition for this case.
\begin{figure}[h]
\begin{minipage}[t]{7.5cm}
\includegraphics[width=0.95\textwidth]{h12a.eps}
\end{minipage}
\hfill
\begin{minipage}[t]{7.5cm}
\includegraphics[width=0.95\textwidth]{h18a.eps}
\end{minipage}
\hfill
\begin{minipage}[c]{7.5cm}
\includegraphics[width=0.95\textwidth]{h24a.eps}
\end{minipage}
\hfill
\begin{minipage}[c]{7.5cm}
\includegraphics[width=0.95\textwidth]{h36a.eps}
\end{minipage}
\caption{Energy histograms for lattice sizes a) $L=12$, b) $L=18$, c) $L=24$, and d) $L=36$ for $q=3$, $J<0$.}
\label{fig:hq3}
\end{figure}\\[1.5mm]
%
\indent
The results shown in the present subsection correspond well with the values reported by Wang and Southern \cite{Wang}. The transition
temperature reported by them is $T_c=0.445$ and their histograms present a behaviour identical to ours.
\clearpage
\subsection{$q=3$, $J>0$:  Ferromagnetic Case}

In this case, the used lattice sizes are $L=18$, $24$, $30$, $36$, $48$, $54$ and $60$. We considered a larger number of lattice sizes in order
to have more points available to estimate the critical exponents. The number of Monte Carlo steps used to thermalize was  $2 \times 10^{5}$, and
the number of steps for averaging was $6 \times 10^{5}$. Binder cumulants of the order parameter $m$ as a function of temperature for
the various $L$ values demonstrated that the system undergoes a second order transition. This is presented in Fig. 1.14. The critical
temperature is obtained from the intersection of all curves, each curve corresponding to a distinct lattice size. The obtained value for the
critical temperature is $T_c = 1.2275$. In Fig. 1.15, specif\mbox{}ic heats for different values of $L$ are shown.\\
\begin{figure}[h]
\begin{minipage}[b][3.2cm][s]{5.4cm}
\caption{Magnetization cumulant showing second order transition at $T_c = 1.2275$. ($q=3$, $J>0$).}
\end{minipage}
\hfill
\begin{minipage}[c]{10cm}
\includegraphics[width=0.92\textwidth]{cumuma.eps}
\end{minipage}\\
\begin{minipage}[b][3.3cm][s]{5.4cm}
\caption{Specif\mbox{}ic heats for distinct lattice sizes for $q=3$, $J>0$.}
\end{minipage}
\hfill
\begin{minipage}[c]{10cm}
\includegraphics[width=0.92\textwidth]{ce2q3a.eps}
\end{minipage}
\end{figure}\\[6.5mm]
%
\indent
We used finite size scaling techniques (see section 1.9) to calculate the critical exponents. To obtain $\nu$, for example, we calculated
the logarithmic derivative of the magnetization in a range near the critical temperature for all lattice sizes selected, and the maximum value
obtained for each curve was plotted against lattice size in a log-log plot. A line was fitted to these points, and its slope gave an estimate of the
value of $1/\nu$. Fig. 1.16 illustrates the procedure. It is important to note that logarithmic derivatives of higher orders of magnetization can be
also used to obtain estimations of $1/\nu$.\\
\begin{figure}[h]
\begin{center}
\resizebox{10cm}{!}{\includegraphics{q3v1a.eps}} \caption{Values of
the logarithmic derivatives of the magnetization for different sizes
of Betts lattice versus the logarithm of $L$. The slope of the
fitted line $y$ gives the value of $\nu$ for $q=3$.}
\end{center}
\end{figure}\\[6.5mm]
\indent
To calculate $\alpha$, the quantities plotted as functions of lattice sizes are the maximum values of specif\mbox{}ic heat  $C_v$. Again, a
linear fit gives the value of $\alpha/\nu$, from which $\alpha$ can be estimated using the value of $\nu$ obtained earlier. The data and the
linear fit are shown in Fig. 1.17.\\
\begin{figure}[h]
\begin{center}
\resizebox{10cm}{!}{\includegraphics{alpha3a.eps}}
\caption{Log-log plot of the maximum values of $C_{\rm V}$ for distinct sizes of Betts lattices. The f\mbox{}it gives the value
of $\alpha/\nu$ for $q=3$.}
\end{center}
\end{figure}

\clearpage The critical exponent $\beta$ is extracted from the
magnetization values at the critical temperature suggested by the
Binder cumulant of magnetization. The logarithm of these values
(remember that each value corresponds to a lattice size) are plotted
versus the logarithm of $L$, and the slope of the line fitting the
data corresponds to $-\beta/\nu$. If instead, the maximum values of
the susceptibility are plotted versus $L$, the critical exponent
$\gamma$ is obtained using the same procedure. (see Figs. 1.18 and
1.19).

\begin{figure}[h]
\begin{center}
\resizebox{9.7cm}{!}{\includegraphics{beta3a.eps}}
\caption{Logarithms of magnetization at the $T_c$ value suggested by
the magnetization cumulant versus logarithms of $L$ values. The fit
gives $-\beta/\nu$ for $q=3$.}
\end{center}
\end{figure}
\begin{figure}[h]
\begin{center}
\resizebox{9.7cm}{!}{\includegraphics{gama3a.eps}}
\caption{Logarithms of susceptibility at the critical temperature
versus logarithms of different linear sizes $L$. The fit gives
$\gamma/\nu$ for $q=3$.}
\end{center}
\end{figure}

\clearpage

One of the common procedures used to obtain the transition temperature consists in plotting the temperature at which the logarithmic derivatives
of the magnetization for each lattice size have their maxima versus $L^{-1/\nu}$. A line is fit to the data and the intersection of this line with
the $y$-axis gives an approximate of the true transition temperature. This can be seen in Fig. \ref{fig:tc3} from which one
gets $T_c=1.22676$.\\[1.5mm]
%
\indent
\begin{figure}[h]
\begin{center}
\resizebox{10cm}{!}{\includegraphics{tc3a.eps}}
\caption{Estimation of the transition temperature $T_c$ ($q=3$, $J>0$).}
\label{fig:tc3}
\end{center}
\end{figure}

In the next table, the critical exponents calculated by Wang and
Southern \cite{Wang}, the values obtained in this work, and the
theoretical values are summarized. The values obtained with the
Monte Carlo simulations agree well to the 2D Potts classical values,
but are not perfectly equal. This can be due to numerical errors,
lattice size effects and also because the Betts lattice can be seen
as a triangular lattice with a large number of defects. Something
that is not so clear to us is why values obtained with the Wolff
algorithm are less similar to the universal values than those
calculated by Wang and Southern.
\begin{table}[h]
\begin{center}
\begin{tabular}{| c || l | l | l |}
\hline
             &  Wang \& Southern Results        & Our Results        & Theory\\
\hline\hline
$\alpha/\nu$ & $0.42\pm0.04$   & $0.464068\pm0.00479$  &$0.4$ \\
\hline
$\beta/\nu$  & $0.132\pm0.002$ & $0.118885\pm0.000203$ &$0.13333$ \\
\hline
$\gamma/\nu$ & $1.74\pm0.05$   & $1.76294\pm0.01072$   &$1.73333$\\
\hline
$1/\nu$      & $1.19\pm0.02$   &$1.20723\pm0.004891$   &$1.2$ \\
\hline
\end{tabular}
\caption{Comparison of the reported critical exponent values with the universal values predicted for the $q=3$ 2D-Potts model.}
\end{center}
\end{table}

\clearpage

\subsection{$q=4$, $J>0$:  Ferromagnetic Case}

The used lattice sizes are once again in the range $L=18$ to $L=60$.
The number of Monte Carlo steps used to thermalize is  $2 \times
10^{5}$, and the number of steps for averaging is $6 \times 10^{5}$.
The Binder cumulant of the order parameter $m$ as a function of
temperature shows that the system undergoes a second order
transition, and it is displayed in Fig. 1.21. The critical
temperature is obtained from the intersection of all curves, each
curve corresponding to a distinct lattice size, and is near
$T_c=1.126$.  In Figs. 1.22 and 1.23, specif\mbox{}ic heats and
susceptibilities for different values of $L$ are shown.
\begin{figure}[h]
\begin{minipage}[b][3.0cm][s]{5.5cm}
\caption{The Binder magnetization cumulant for $q=4$, $J>0$.}
\end{minipage}
\begin{minipage}[c]{9.7cm}
\includegraphics[width=0.92\textwidth]{cumum4a.eps}
\end{minipage}
\hfill
\begin{minipage}[b][3.0cm][s]{5.5cm}
\caption{Specif\mbox{}ic heats for different lattice sizes ($q=4$, $J>0$).}
\end{minipage}
\begin{minipage}[c]{9.7cm}
\includegraphics[width=0.92\textwidth]{ce2q4a.eps}
\end{minipage}
\hfill
\begin{minipage}[b][3.0cm][s]{5.5cm}
\caption{Susceptibilities for different lattice sizes ($q=4$, $J>0$).}
\end{minipage}
\hfill
\begin{minipage}[c]{9.7cm}
\includegraphics[width=0.92\textwidth]{susce4a.eps}
\end{minipage}
\hfill
\end{figure}\\[6.5mm]
\indent
The critical exponents were obtained with the same procedures explained for $q=3$. Different thermodynamic quantities are calculated for each
lattice size, and the values near critical temperature are plotted against linear size in various log-log plots. A line is fit to the data and its
slope is representative of some critical exponent, depending on which thermodynamic quantity was selected to be plotted (Fig. 1.24 to Fig. 1.27). The
critical temperature is estimated in the same way explained earlier, and is shown in Fig. 1.28.\\
\begin{figure}[h]
\begin{minipage}[b][3.0cm][s]{4.5cm}
\caption{Values of the logarithmic derivatives of magnetization for
different sizes of Betts lattice, versus logarithm of $L$. The fit
gives the value of $1/\nu$ for $q=4$, $J>0$.}
\end{minipage}
\begin{minipage}[c]{10cm}
\includegraphics[width=0.92\textwidth]{q4v1a.eps}
\end{minipage}
\hfill
\begin{minipage}[b][3.0cm][s]{4.5cm}
\caption{Logarithm of the maximum value of $C_v$ for different sizes
of Betts lattice, versus logarithm of $L$. The fit gives the value
of $\alpha/\nu$ for $q=4$, $J>0$.}
\end{minipage}
\hfill
\begin{minipage}[c]{10cm}
\includegraphics[width=0.92\textwidth]{alpha4a.eps}
\end{minipage}
\hfill
\end{figure}

\clearpage

\begin{figure}[h]
\begin{minipage}[c]{9.7cm}
\includegraphics[width=0.92\textwidth]{beta4a.eps}
\end{minipage}
\begin{minipage}[b][3.0cm][s]{4.5cm}
\caption{Logarithms of the magnetization values at the critical
temperature of various lattice sizes versus logarithms of $L$. The
fit gives $-\beta/\nu$ for $q=4$, $J>0$.}
\end{minipage}
\hfill
\begin{minipage}[c]{10.0cm}
\includegraphics[width=0.92\textwidth]{gama4a.eps}
\end{minipage}
\hfill
\begin{minipage}[b][3.0cm][s]{4.5cm}
\caption{Logarithms of the susceptibilities at the critical
temperature of various lattice sizes versus logarithms of $L$. The
fit gives $\gamma/\nu$ for $q=4$, $J>0$}
\end{minipage}
\hfill
\begin{minipage}[c]{10.0cm}
\includegraphics[width=0.92\textwidth]{tc4a.eps}
\end{minipage}
\hfill
\begin{minipage}[b][2.5cm][s]{4.5cm}
\caption{Estimation of the critical temperature for $q=4$, $J>0$.}
\end{minipage}
\hfill
\end{figure}

\clearpage


The values obtained for the critical exponents are summarized in the next table, along with the theoretical values expected. The value obtained
for $\beta$ is not near the expected value, and this can be due to an effect of magnetic frustration on the lattice. More calculations need to
be done in the future, with larger lattice sizes, however it could be that this lattice does not belong to an universal group.

\begin{table}[h]
\begin{center}
\begin{tabular}{| l || r | r | c |}
\hline
             & Our Results                    & Theory \\
\hline\hline
$\alpha/\nu$ & $0.644537\pm0.03695$  & $1$ \\
\hline
$\beta/\nu$  & $0.0562526\pm0.004001$& $0.125$ \\
\hline
$\gamma/\nu$ & $1.75564\pm0.02506$ &  $1.75$ \\
\hline
$1/\nu$      & $1.38519\pm0.03172$ & $1.5$ \\
\hline
\end{tabular}
\caption{Comparison of critical exponent values obtained by us with the universal values predicted theoretically for $q=4$ 2D-Potts model.}
\end{center}
\end{table}

\subsection{$q=5$, $J>0$:  Ferromagnetic Case}

The lattice sizes considered once again are in the range $L=18$ to $L=60$. The number of Monte Carlo steps used to thermalize is $2 \times 10^{5}$,
and the number of steps for averaging is $6 \times 10^{5}$. The Binder cumulant of the order parameter $E$ as a function of temperature suggests that
the system undergoes a first order transition, and it is presented in Fig. 1.29. The critical temperature is obtained from the deep of all curves,
each curve corresponding to a different lattice size, and is near $T_c=1.0575$. Specific heats are shown in Fig. 1.30.\\[1.5mm]
%\begin{figure}[h]
%\begin{center}
%\begin{minipage}[c]{10.0cm}
%\includegraphics[width=0.99\textwidth]{cumue5a.eps}
%\end{minipage}
%\begin{minipage}[b][2.1cm][s]{4.0cm}
%\caption{Energy cumulant for $q=5$, $J>0$. The transition temperature is near 1.0575.}
%\end{minipage}
%\begin{minipage}[c]{10.0cm}
%\includegraphics[width=0.99\textwidth]{ce1q5a.eps}
%\end{minipage}
%\begin{minipage}[b][2.1cm][s]{4.0cm}
%\caption{Specif\mbox{}ic heats for $q=5$, $J>0$.}
%\end{minipage}
%\end{center}
%\end{figure}\\[1.5mm]
%
\indent
For the calculation of energy histograms, the number of Monte Carlo steps used for thermalization is  $1 \times 10^{6}$, and the number of steps
for averaging varies from  $3 \times 10^{6}$ for lattice sizes until $L=36$, and $4 \times 10^{6}$ for the next lattice sizes. The results are shown
in Fig. 1.31.\\[1.5mm]
%
\indent
Energy histograms conf\mbox{}irm that the transition is f\mbox{}irst order. The histograms are narrow at increased lattice size, and the valleys also become deeper.\\

\begin{figure}[h]
\begin{center}
\resizebox{10cm}{!}{\includegraphics{cumue5a.eps}}
\caption{Energy cumulant for $q=5$, $J>0$. The transition temperature is near 1.0575.}
\end{center}
\end{figure}
\begin{figure}[h]
\begin{center}
\resizebox{10cm}{!}{\includegraphics{ce1q5a.eps}} \caption{Specific
heats for $q=5$, $J>0$.}
\end{center}
\end{figure}

\begin{figure}[h]
\begin{minipage}[t]{7.5cm}
\includegraphics[width=0.92\textwidth]{q5h18a.eps}
\end{minipage}
\hfill
\begin{minipage}[t]{7.5cm}
\includegraphics[width=0.92\textwidth]{q5h24a.eps}
\end{minipage}
\hfill
\begin{minipage}[t]{7.5cm}
\includegraphics[width=0.92\textwidth]{q5h30a.eps}
\end{minipage}
\hfill
\begin{minipage}[t]{7.5cm}
\includegraphics[width=0.92\textwidth]{q5h36v2a.eps}
\end{minipage}
\hfill
\begin{minipage}[t]{7.5cm}
\includegraphics[width=0.92\textwidth]{q5h48v2a.eps}
\end{minipage}
\hfill
\begin{minipage}[t]{7.5cm}
\includegraphics[width=0.92\textwidth]{q5h54a.eps}
\end{minipage}
\hfill
\begin{minipage}[t]{7.5cm}
\includegraphics[width=0.92\textwidth]{q5h60a.eps}
\end{minipage}
\hfill
\begin{minipage}[b][2.9cm][s]{6.2cm}
\caption{Energy histograms for lattice sizes a) $L=18$, b) $L=24$, c) $L=30$, d) $L=36$, e) $L=48$, f) $L=54$ and g) $L=60$.}
\end{minipage}
%\label{fig:hiq5}
\end{figure}

\clearpage

\subsection{Conclusion}

The results obtained with Monte Carlo simulations and finite size scaling techniques show clearly the kind of transition for each of the cases
presented. The calculated critical exponents were near the theoretical values for second order phase transitions, except for the
exponent $\beta$ in the case $q=4$ that requires a more detailed analysis. Remember that for $J>0$ the transition is supposed to be of second
order for $q \leq 4$ and of first order for $q > 4$. As it lies at the border between the two, the case $q=4$ is difficult to assess. Another
aspect that must be taken into account for further analysis is the type of lattice, because it is quite probable that magnetic frustration
effects could modify the magnetization-related critical coefficients. For first order transitions, the values of the free energy barriers could
be estimated from the difference between the two peaks and the valley.\\[1.5mm]
%
\indent
As we mentioned at the end of section 1.1, Monte Carlo simulations are a helpful tool in other areas. Thus, in the next chapter
we will move on and review a cluster identification technique that involves Monte Carlo calculations for the analysis of biological data.

